Combinatorial Pure Exploration with Full-bandit Feedback and Beyond: Solving Combinatorial Optimization under Uncertainty with Limited Observation

Combinatorial optimization is one of the fundamental research fields that has been extensively studied in theoretical computer science and operations research. When developing an algorithm for combinatorial optimization, it is commonly assumed that parameters such as edge weights are exactly known as inputs. However, this assumption may not be fulfilled since input parameters are often uncertain or initially unknown in many applications such as recommender systems, crowdsourcing, communication networks, and online advertisement. To resolve such uncertainty, the problem of combinatorial pure exploration of multi-armed bandits (CPE) and its variants have recieved increasing attention. Earlier work on CPE has studied the semi-bandit feedback or assumed that the outcome from each individual edge is always accessible at all rounds. However, due to practical constraints such as a budget ceiling or privacy concern, such strong feedback is not always available in recent applications. In this article, we review recently proposed techniques for combinatorial pure exploration problems with limited feedback.

==> sec/abstract.tex <==

%\chapter*{Abstract}
\addcontentsline{toc}{chapter}{Abstract}
%テキーラ大好き。


% What is the reason for writing the thesis?
% What are the current approaches and gaps in the literature?
% What are your research question(s) and aims?
% Which methodology have you used?
% What are the main findings?
% What are the main conclusions and implications?
%日常の組合せオンライン学習の応用の話
%組合せ最適化の不確実性とも関わってる話，
%multi-armed bandit
%
% Decision making under uncertainty in humans has been investigated in several psychological, neuroimaging and neuropsychological studies

%Sequential decision making under uncertainty is a 
% Human beings are constantly exposed to uncertainty situations in which the careful weighing of possible outcomes is required to make decisions.
\begin{eabstract}

\emph{Decision making under uncertainty} is common in prudent weighing of outcomes or utility because we human beings are constantly exposed to risk or ambiguity situations. In the face of uncertainty in our lives,
we aim to take the best possible decision based on the past experience and conjecture. Modeling of decision making under uncertainty and its analysis have been investigated in diverse research fields such as computer science, statistics, psychology, and neuroscience.

The problem of \emph{stochastic multi-armed bandits} is one of the classical decision making models, and it lies at the intersection of statistics and machine learning.  The stochastic multi-armed bandit problem characterizes the trade-off between exploration and exploitation in stochastic environments; in this problem, an agent chooses one action (a.k.a.~arm) from $K$ given arms at each step, and obtains a reward sampled from an unknown probability distribution associated with the chosen arm.

 In many real-world scenarios, our decisions are often characterized by a combinatorial and complex structure. For example, possible actions in real-world systems may be a subset of keywords in online advertisements, assignments of tasks to workers in crowdsourcing, or paths in communication networks．The problem of \emph{stochastic combinatorial bandits} is a generalization of the multi-armed bandits, which can deal with such combinatorial actions; a subset of arms (a.k.a~super arm) is an action in this model, while each single arm is an action in the multi-armed bandit problem.

 In this thesis, we study stochastic combinatorial bandit problems from an algorithmic perspective. 
Motivated by real-world applications, we develop theory and algorithms for challenging settings, in which only limited feedback is given to an agent.
In the combinatorial bandit literature, a large amount of work has studied the \emph{semi-bandit} setting, in which an agent can directly observe a random feedback from an individual arm at each sampling trial.
However, such a sampling procedure for individual arms is costly or often impossible due to the privacy issues or system constraints.
To overcome this critical limitation of existing studies,
we aim to propose statistically and computationally efficient methods based on only limited observation. To this end, we address several approximation algorithms for NP-hard problems and bandit algorithms that can deal with an aggregated feedback from a super arm.


This thesis focuses on the combinatorial bandit problems in the \emph{pure exploration} setting;
in this setting, an agent aims to identify the optimal super arm with the highest expected reward.
The learning performance is evaluated by the number of samples required by her learning algorithm, i.e., the \emph{sample complexity}, rather than the cumulative rewards.
The main body of this thesis consists of four parts,
which corresponds to Chapters 3--6.
The first part is devoted to a study of pure exploration for top-$k$ arms with \emph{full-bandit feedback}, where underlying combinatorial structures are simply size-$k$ subsets but available feedback is limited to a noisy evaluation for a sampled subset of arms, i.e., full-bandit feedback.
The second part is devoted to a study of general combinatorial pure exploration with full-bandit feedback, in which possible combinatorial structures are size-$k$ subsets, matchings, and paths.
The third part is devoted to a study of combinatorial pure exploration over graphs with full-bandit feedback, which aims to identify a dense component in a network only together with a noisy evaluation for a sampled subgraph.
The fourth part is devoted to a study of general combinatorial pure exploration with \emph{partial-linear feedback}, which aims to develop a novel algorithmic framework for general (possibly nonlinear) reward functions and combinatorial structures including size-$k$ subsets, matchings, and paths.
Partial-linear feedback ranges from semi-bandit and full-bandit feedback;
in this feedback model, the agent only observes a linear combination of rewards of the chosen super arm at each pull.

In Chapter~3, we first investigate a novel problem of pure exploration for top-$k$ arms  with full-bandit feedback. Although our problem can be regarded as an instance of linear bandit problems, a naive approach using linear bandit algorithms is computationally infeasible to the problem instance in the combinatorial setting, since the number of possible actions $K$ is exponential with respect to the number of arms in the subset. To cope with this problem, we design a polynomial-time approximation algorithm for the 0-1 quadratic programming problem arising in confidence ellipsoid maximization. Based on our approximation algorithm, we propose a bandit algorithm whose time complexity is $O(\log K)$, thereby achieving an exponential speedup over linear bandit algorithms. We also provide an upper bound on the sample complexity that is worst-case optimal. Our experiments on large-scale crowdsourcing datasets with more than $10^{10}$ possible actions demonstrate the superiority of our algorithm in terms of both the computation time and the sample complexity.

 In Chapter~4, we study combinatorial pure exploration with
full-bandit feedback for general combinatorial structures such
as matroids, matchings, and $s$-$t$ paths.
We devise a polynomial-time adaptive algorithm whose sample complexity has mild dependence on the \emph{minimal gap} between the optimal value and the second optimal value. 
We show that the sample complexity  matches (within a logarithmic factor) the information theoretic lower bound for a family of instances.
We conduct a series of experiments on the matching and top-$k$ instances and demonstrate that (a) the proposed algorithm scales to combinatorial instances while existing linear bandit algorithms require a prohibitive amount of time; (b) the number of samples required by the proposed algorithm is not sensitive to the value of the minimum gap.

 In Chapter~5, we focus on a specific instance of combinatorial pure exploration with linear feedback over graphs with applications to \emph{dense subgraph discovery under uncertainty}. We introduce a novel learning problem for online dense subgraph discovery, in which an agent queries subsets of edges rather than single edges and observes a noisy sum of edge weights in a queried subset. For this problem, we propose a polynomial-time algorithm that obtains a nearly-optimal solution with high probability. For the proposed algorithm, we provide an upper bound of the number of samples that the algorithm requires.
Moreover, to deal with large-sized graphs, we design a more scalable algorithm that maximizes the quality of solution within a fixed number of queries.
Computational experiments using real-world graphs demonstrate the effectiveness of our algorithms.

In Chapter~6, we study a novel model of general combinatorial pure exploration with partial-linear feedback, which includes all the problems addressed in Chapters~3--5 as special cases and finds various applications such as online ranking in recommendation systems and crowdsourcing. The model of partial-linear feedback fits in such real-world applications since it may happen that we cannot always observe outcomes from some of the chosen arms due to privacy
concern or system constraints. We propose a polynomial-time algorithmic framework for this general problem, and provide a sample complexity analysis.

 To summarize, we investigate the learnability of the combinatorial pure exploration problems with limited feedback and develop polynomial-time algorithms. Our results provide novel insights into online decision making problems with combinatorial action spaces and combinatorial optimization under uncertainty for incomplete inputs.


\end{eabstract}

\begin{jabstract}
我々人間は，予想不可能な事態，危険性に常に晒されながら，意思決定を行なっている．
我々は不確実な事象を前にして，過去の経験や推測に基づいて最善な意思決定を下そうとする．
そのような\textbf{不確実性の下での意思決定}は,
より良い結果を得るために重要な営みである．
不確実性を伴う意思決定のモデル化とその分析は，情報科学，統計学，心理学，神経科学など幅広い学術分野で古くから議論されてきた．

\textbf{確率的多腕バンディット問題}は古典的な意思決定モデルの一つであり，統計学と機械学習の共通領域に位置している．
この問題では，エージェントは$K$個の行動候補からただ一つの行動を各時刻で選択しなければならない．そして，選択した行動により(確率的な)報酬を得るが，選択しなかった行動からの報酬は観測不可能であり，ここに探索と活用のジレンマが生じている．

我々の意思決定は組合せ的な意思決定がほとんどである．
例えば，オンライン広告におけるキーワードの選択や，労働者とタスクの割当，通信ネットワークにおける経路などは，組合せ的な意思決定問題である．
\textbf{確率的組合せバンディット問題}では，各行動がある組合せ的構造を持っている行動を扱っており，この問題は上記の確率的多腕バンディット問題の一般化となっている．

本学位論文では，
%アルゴリズム論的観点から組合せバンディット問題について探求する．
実世界の状況をより忠実に扱うために，
限られた観測しか得られない挑戦的な設定における組合せバンディット問題に対するモデル化とアルゴリズム設計を目指す．
既存研究の主流では，\textbf{半バンディット}と呼ばれる選択した行動に含まれる各要素を個々に直接観測する場合が扱われてきた．
しかし，実世界の問題では，プライバシー保護や実応用上の制約，コストの観点から，そのような個々に関する観測を得ることは難しく，現実的な設定とは言えない．
本研究ではこのような既存研究の枠組みの問題を解決すべく，理論と応用の両側面から良い性質を持った手法の開発を目標とする．
この目標に向けて，いくつかのNP困難な最適化問題に対する近似アルゴリズムの設計を提案するとともに，いかにして限られた観測情報を扱うかを議論し，統計的かつ計算量的に良い性質を持つ汎用性の高いアルゴリズム開発を目指す．

組合せバンディット問題の中でも，\textbf{最適腕識別}と呼ばれる枠組みに焦点を当てる．最適腕識別問題は期待報酬が最大となる行動を見つける問題で，アルゴリズムの評価指標は累積報酬ではなく，出力までに用いた標本数，つまり\textbf{標本複雑度}が用いられる．
本学位論文の主結果は第三章から第六章までの四つの章で議論されている．第三章では限定的な観測に基づく組合せ最適腕識別問題の中でも最も単純な問題である，線形の重み和が最大となるサイズ$k$の集合を求める問題を扱う．ここで観測として得られるのは，選択した集合からのノイズありの重み和のみである．この観測形態を，半バンディット観測に対して\textbf{全バンディット}観測と呼ぶ．
第四章ではマトロイド，マッチング，パスなど幅広い組合せ制約にも適用可能なアルゴリズムを提案する．
第五章ではグラフ上における最も密な部分グラフを検出することを目的とした，グラフ上の組合せ最適腕識別問題を扱う．
第六章では\textbf{部分観測}と呼ばれる，半バンディットや全バンディットを特殊ケースとして含む観測形態を扱う設定を議論する．さらに報酬関数として非線形関数を扱える一般的な解法を提案する．以下にそれぞれの主結果を述べる．


第三章では，サイズ$k$集合を求める全バンディット組合せ最適腕識別問題を扱う．この問題では，各時刻にサイズ$k$集合を一つ選択したあとその確率的な重み和を観測し，
なるべく少ない標本数で最適なサイズ$k$集合を求めることを目指す問題である．
%アルゴリズムが必要とする標本数の上界を\textbf{標本複雑度}と呼ぶ．
既存の線形モデル上の最適腕識別問題への解法は，その計算量が全ての候補数に線形に依存するため，組合せの設定に対しては指数時間アルゴリズムとなってしまう．本研究では二次計画問題として定式化される信頼区間最大化に対して多項式時間近似アルゴリズムを設計し，計算量的にも統計的にも効率的なアルゴリズムを開発する．
クラウドソーシングを用いた計算機実験でその有効性を検証する．

第四章では，
サイズ，マトロイド，$s$-$t$ パス，マッチングなどを含む一般的な組合せ制約を扱える枠組みを提案する．
第三章での提案手法が静的サンプリング戦略に基づいていたのに対し，本章では組合せ構造を利用した動的なサンプリング戦略に基づくアルゴリズムを設計する．
動的なサンプリング戦略により，標本数の上界が最適値と次に良い値の差への依存度を軽減できることを理論的に示し，計算量および統計的に妥当であることを計算機実験により示す．



第五章では，
最密部分グラフ抽出問題の全バンディット観測設定を扱う．
既存手法のように毎回一本の枝からの観測を得るのではなく，枝集合からの重み和のみが観測される設定を考える．この問題に対し，高確率で最適解を求める多項式時間アルゴリズムを提案し，その標本複雑度を理論的に解析する．さらに，標本数があらかじめ決まっている設定に対して，貪欲法に基づく効率的なアルゴリズムを設計し，1/2近似解を出力する確率の下界を示す．
実グラフを用いた計算機実験により提案手法の妥当性を示す．

第六章では，
% サイズ，マトロイド，$s$-$t$ パス，マッチングなどを含む一般的な組合せ制約を扱える枠組みを提案する．
% 組合せ構造を利用した動的なサンプリング戦略に基づく計算効率の良いアルゴリズムを設計する．標本数の上界が最適値と次に良い最適値の差への依存が少ないことを理論的に示し，統計的にも妥当であることを保証する．
% さらに，
非線形報酬関数と部分観測を同時に扱えるより一般的なモデルを提案する．
推薦システムやクラウドソーシングといった実応用では，プライバシー保護やシステムの制約上，必ずしも選んだ集合に対する観測が得られるとは限らず，部分集合に対する観測しか得られない状況があり得る．また，報酬が線形ではない設定も多く存在する．
そのような場合にも適応可能な多項式時間アルゴリズムを提案し，アルゴリズムが最適解を出力するのに必要な標本数の上界を示す．


以上を要するに，本学位論文では，限定的な観測に基づく組合せ最適腕識別問題に対する多項式時間アルゴリズムによる学習可能性を示し，組合せ構造を扱う複雑なオンライン意思決定問題や，入力が不完全な場合の不確実性を伴う組合せ最適化問題に対して新たな洞察を与えた．

% 最後に今後の展望を述べる．
% さらなる理論限界の解明のために，
% 本研究で扱った全バンディットや部分観測に基づく最適腕識別問題への多項式時間アルゴリズムが必要な標本数の下界の証明は重要な課題である．
% さらに，観測が非線形である場合や報酬関数が非定常である場合への拡張も，実応用上開発すべき課題である．
% また，組合せ最適腕識別問題と，推定誤差を最小化するためのサンプル集合を求める\textbf{実験計画問題}は密接に関わっている．さらなる標本複雑度の改善に向けて，組合せ制約を扱える実験計画問題へのアルゴリズム開発も重要な課題であろう．


\end{jabstract}

==> sec/acknowledge.tex <==
\chapter*{Acknowledgments}
\addcontentsline{toc}{chapter}{Acknowledgments}

%Thank you all :)

First and foremost, I would like to express my deepest gratitude to my supervisor Professor Masashi Sugiyama, for his guidance and patience throughout my PhD.
I first learned about him when I came across his book at Tokyo Institute of Technology, and it invited me to
a fascinating world of machine learning.
I was very lucky to join his laboratory from the PhD program
and learned a lot from him and his group.
He had a great influence on me and sharpened my research mind indeed.
Thanks to him, I had opportunities to meet many wonderful students and researchers coming from around the world, which was a great experience for me.
Through my difficult times,
he always managed to make time and supported me despite his extremely busy schedule.
His hard work and enthusiasm for research have been my great inspiration,
and encouraged me to pursue a career in research.
For that, I am forever grateful to him.

I would also like to express my sincere gratitude to my another advisor
Senior Lecturer Junya Honda,
for his continuous assistance to my research.
He kindly spent a great deal of time supporting me from the beginning of research projects throughout the paper writing or presentation stages.
His technical assistance was especially helpful and necessary to complete my research.
Without his careful and thoughtful guidance, my PhD would not have been achievable in any sense.

Also, 
I am very thankful to Associate Professor Issei Sato, Senior Lecturer Naoto Yokoya,
Dr.~Ikko Yamane,  Dr.~Yoshihiro Nagano,
and the secretary Ms. Yuko Kawashima for their constant support to maintain the research environment.
In paticular, Associate Professor Issei Sato provided me with
valuable advice for not only research, but also life.
I deeply appreciate their help.

My special thanks are due to Professor Wei Chen at Microsoft Research Asia,
who is one of the pioneers in combinatorial bandits.
I have read many his papers and his work has had great influence on my PhD studies. So I feel extremely lucky for having had the chance to work with him. Although I could not visit his laboratory, 
he has set up discussion every week and advised me remotely from Beijing.
Also, I would like to thank Ms.~Yihan Du at Tsinghua University,
who is the other collaborator in MSRA projects.
Besides the regular meetings, I have always discussed with her by WeChat and her hard work has motivated me to continue working on research even when we got stuck.
Chapters~\ref{chap:CPE-BL} and~\ref{chap:CPE-PL} are based on the joint work with them, and I cannot thank them enough for their collaboration. I really want to meet them someday.

The collaboration research with MSRA came true thanks to Ms.~Mawo Kamakura,
Research Program Manager at Microsoft Research.
She frankly communicated with me and gave me confidence.
She also connected me to some Japanese female students in computer science, which was really helpful for me.

I would like to thank the other collaborators, Assistant Professor Atsushi Miyauchi and Mr. Liyuan Xu,
for their valuable discussions and helpful comments.
Assistant Professor Atsushi Miyauchi helped me develop theory and algorithms for graph optimization problems.
Mr. Liyuan Xu helped me understand the best arm identification in linear bandits, and my first work of PhD studies is inspired by his paper.


Working at Sugiyama-Sato-Honda (later Sugiyama-Honda-Yokoya) Lab was one of the most wonderful time in my life. I
thank all the present and past members of the laboratory for the pleasant atmosphere.
In the last three years, I have enjoyed not only research but also many activities including playing badminton or tennis, playing board games or cards, going to the beach, finding for good beer and nice restaurants, and everything.
I am especially thankful to Kento Nozawa, Nontawat Charoenphakdee,
Han Bao, Liyuan Xu, Takeshi Teshima, Jongyeong Lee, Taira Tsuchiya, Zijian Xu, Dr.~Ikko Yamane, Dr.~Futoshi Futami, Seiichi Kuroki, Chenri Ni, and Hideaki Imamura.  They have all helped me keep smiling, laughing and happy.
I will never forget the wonderful time spent with all the lab members.


Last, but not least, I wish to thank my family for their love and support.
I dedicate this thesis to my late grandfathers,
whose dream was to see me complete my PhD.






% Cleveland during most of my training at CMU, but he has never failed to provide me
% with enough resources, readings to follow, time for discussions and advice.
% % Associate Professor Dr.Vanida Durongrittichai, and Kanokwan Chanthanamongkol,
% lecturer of Faculty of Nursing in Huachiew Chalermprakiet University for their
% encouragement and support.
% connected to many researchers

% His enthusiasm for research, his passion for life,
% and his work ethic e and will continue to shape
% me in the future.
% Christos has been the best advisor anyone could hope for. He always cares for his students not only academically
% but also personally. In every project, Christos was always there from the brainstorming stage throughout the detailed technical discussions and to the paper writing and presentation stages. After five years of working with him, his ways of academical thinking and writing styles have been adopted to me. Apart from research,
% Christos would also make sure that I am feeling well, balancing work and life. Christos has provided me with an opportunity to explore various research topics, which
% helped me learn a lot in broad scope of applications. I was fortunate to be given
% a great opportunity to collaborate with smart colleagues within and outside CMU
% (University of Pittsburgh, University of Minnesota, University of Virginia, University of Porto, Data Insights Laboratories) and also within and outside SCS (ECE,
% Statistics, Informatics). This wide collaboration across departments and schools has
% been one of the fun experiences I had in my PhD program. I will always remember
% his endless passion for various research topics and positivity, as well as his passion
% for pictionary, charades, and jokes at the group parties. efcharisto (thanks)!
% First and foremost, I am greatly indebted to my advisor, Geoff Gordon, who, throughout
% my five-year journey at Carnegie Mellon University, has provided me with constant supports,
% insightful discussions, as well as the freedom that allows me to pursue interesting research
% problems to fulfill my own curiosity. In addition to being a fantastic researcher, Geoff is also
% the kindest and most supportive individual that I have had the pleasure of working with. He
% has a great sense of research taste, which also shapes mine to work on important and elegant
% questions. I would like to sincerely thank Geoff for his intuitive insights in understanding
% complex problems, for sharing with me his broad knowledge in almost every aspect of machine
% learning, and for his unwavering faith in me that pushes me to become a better researcher. I
% hope that I could become a researcher, an advisor and a person like him in the future
% Undertaking Ph.D at CMU has been a truly life-changing experience for me. It requires
% me to fully make a commitment to myself more than ever before. However, it would not
% have been possible to do without the support and guidance that I received from many people.
% Firstly, I would like to express my deepest gratitude to my advisor Prof. Edward
% Kennedy for the continuous support of my Ph.D studies and related research, for his patience,
% motivation, and for his immense knowledge of statistics. Having him as my Ph.D advisor is
% the luckiest thing that ever happened during my Ph.D studies. He has been supportive since
% the days I began working with him, not only academically but also emotionally through the
% rough road to finish my Ph.D. Without his clear guidance and constant feedback, this Ph.D
% would not have been achievable in any sense. It is whole-heartedly appreciated that his great
% advice for my study proved monumental towards the success of this Ph.D degree. Edward
% was the reason why I decided to go to pursue a career in research.
% I would like to pay my special regards to my another advisor Prof. Larry Wasserman for
% the invaluable assistance that he has provided during my Ph.D studies. He is a genuine expert
% in statistics and machine learning; in many cases, just a few words of his email body are
% enough to make a breakthrough in my research. Most importantly he is a wonderful person.
% I could not have imagined having a better advisor and mentor for my study in statistical
% machine learning.
% Besides my advisors, my sincere thanks also go to the rest of my thesis committee
%. I dedicate this dissertation to my late father, Raghavan Sridharan, whose
%greatest dream was to see me complete my PhD
% I have no doubt on that this dissertation would have been impossible without various support of many people. First of all, I am grateful for my supervisor, Satoru Iwata, who invited me to the world of academic research. He has been continuously giving many research ideas, suggestions, and advice during my Ph.D. program with great patience. My days in the Ph.D. course would have been completely different without his infinite support.
% I also would like to acknowledge that many parts of this dissertation are based on joint works with my collaborators. Especially, I would like to thank Yuichi Yoshida. His endless mathe- matical ideas and great depth of knowledge on computer science have been truly remarkable and inspired me a lot.
% The idea of the first part of this dissertation originates from my first joint project with Naonori Kakimura, Kazuhiro Inaba, Ken-ichi Kawarabayashi. Their research ideas and valuable discussions with them were really helpful and they took me to the research field of machine learning.
% Chapter 8 benefited from many discussions and suggestions of Yuji Nakatsukasa and Andr ́e Uschmajew during our joint work. They raised my small mathematical problem into really fascinating one, invited me to an exciting research area of sparse optimization, and greatly expanded the scope of my research.
% I also would like to thank members and former members of our laboratory, especially Ku- nihiro Sadakane, Akiko Takeda, Yutaro Yamaguchi, Yu Yokoi, Naoki Ito, Shuichi Katsumata, and Kaito Fujii. Their valuable comments in our seminar and supports in my daily life in the laboratory have been really appreciated.
% Furthermore, I would like to thank my parents for their support and love. Spending ten years as a student was not short, but they always encouraged me to continue my research.
% Finally, I thank Japan Society for Promotion of Science, JST ERATO Kawarabayashi Large Graph Project, JST CREST Iwata team, and the University of Tokyo for their financial sup- port.

%First and foremost, I would like to thank my two awesome advisors, Eric Xing
%and Pradeep Ravikumar, who have always been tremendously supportive and
%understanding. I am grateful for the exceptional freedom they allowed, as well
%as the guidance they provided when I was facing difficulties.
%. I am exceedingly grateful to
%Zico for always putting my own development and interests first, patiently guiding me to be a better researcher and humd human being, and believing in my work every step of the way for over seven years.
%m. I will always remember his endless passion for various research topics and positivity, as well as his passion for pictionary, charades, and jokes at the group parties
%n. I owe them both for the many things I have learned in machine learning over the last five years and my personal development as a researcher
% I take this opportunity to express my deepest gratitude and appreciation to my supervisors, Rémi Munos and Alessandro Lazaric. I am extremely grateful for your careful and thoughtful guidance, for your patience and understanding. For your great research insights, vision, enthusiasm, and rigour that you generously shared with me. For your investment and the great help and support you offered me, fundamental to this thesis. I am also thankful for your constant encouragement and kindness. I feel extremely lucky for having had the chance to work with you and learn from you, I cannot thank you enough for it.

% First and foremost, I am greatly thankful to my advisor, Drew Bagnell, who, throughout
% my five years at Carnegie Mellon University, has pointed me to interesting research problems,
% provided me insightful discussions, and gave me freedom to pursuitmy own research
% ideas. Drew himself is an inspiring person. As the CTO of Aurora, he comes to CMU every
% Wednesday to spend time with us to discuss research ideas, read research papers, and give
% advice on our research projects. His desire to learn about new papers, to hunt for new research
% directions, and to understand new research problems, have been motivating me: if a
% busy CTO still has the time and the enthusiasm for research, there will be no excuse for me!
% Drew is a great advisor, a great researcher and a great role model! For that, I am forever
% grateful.
% I would
% I am extremely grateful to my supervisor Professor Masashi Sugiyama for his support,
% patient guidance, enthusiastic encouragement and constructive suggestions
% during my Ph.D. studies. I would also like to express my great appreciation to my
% mentor Dr. Hirotaka Hachiya, who introduced me important ideas of reinforcement
% learning field, gave me valuable advice and productive discussions about my
% research. The most important is that Dr. Hirotaka Hachiya taught me how to do
% research and encouraged me a lot during the toughest time of my studies.
% For investing the usefulness of my proposed method in humanoid robot tasks, a
% lot of thanks to Dr. Jun Morimoto of ATR, kyoto, who provided me the simulator
% of the humanoid robot CBi and introduced me valuable knowledge of robotics.
% Also, I wish to express my gratitude to my college Voot Tangkaratt, who did a
% great job in the humanoid robot experiments.

% First and foremost, I would like to thank my supervisor, Prof. Hiroshi Imai, for
% his precious advice and encouragement from his broad knowledge and experience.
% Without his support and guidance, my four years in graduate school could not be
% accomplished. I am also obliged to him for showing me how to conduct research
% eectively, how to present results in papers and talks, and how to communicate
% with other researchers. These skills would be denitely valuable in my whole
% research career.
% I am also very honored to have Prof. Naoki Kobayashi as the chair, and Prof.
% Masami Hagiya, Prof. Reiji Suda, Prof. Tetsuo Shibuya, Prof. Kunihiko Sadakane,
% and Prof. Satoru Iwata as the members of the committee for this Ph.D. thesis.
% I highly appreciate them taking the time and eort to study and examine this
% thesis.
% I am also profoundly grateful to my great collaborators so far, Christian Sommer,
% Ken-ichi Kawarabayashi, Yoichi Iwata, Yuichi Yoshida, Yosuke Yano, Yuki
% Kawata, Takanori Maehara, Nori Nozomi, and Takanori Hayashi. I really enjoyed
% working with these insightful and talented people, where I learned a lot
% from them.
% I would also like to thank all members in Imai Laboratory, Akitoshi Kawamura,
% Francois Le Gall, Masato Edahiro, Mami Takahashi, Norie Fu, Vorapong
% Suppakitpaisarn, Kenta Takahashi, Hiroyuki Miyata, Toshihiro Tanuma,
% Takahiko Satoh, Jean-Francois Baer, Yoshikazu Aoshima, Akihiro Hashikura,
% Shunichi Matsuda, Ly Nguyen, Yoichi Iwata, Hidefumi Hiraishi, Hiroyuki Ohta,
% Junya Fukawa, Chitchanok Chuengsatiansup, Alonso Gragera, Bingkai Lin, Keigo
% Oka, Akira Motoyama, Yuto Hirakuri, Yuki Kawata, Chihiro Komaki, Yosuke
% Yano, Naoto Ohsaka, Takuto Ikuta, Shuichi Hirahara, Takanori Hayashi, Makoto
% Soejima, Kentaro Yamamoto, Holger Thies, Jeremy Cohen, and Simon Klein.
% In addition to the main laboratory, I also had the privilege of working with or
% visiting several prominent research groups. First, I have been a member of the
% complex network and map graph group at JST ERATO Kawarabayashi Large
% Graph Project. As people there have close research interest with me, I pretty
% enjoyed the weekly seminar with them, specically, Ken-ichi Kawarabayashi,
% Yuichi Yoshida, Naoki Masuda, Takehisa Hasegawa, Kazuhiro Inaba, Yutaka
% Horita, Ryosuke Nishi, Junichi Teruyama, Taro Takaguchi, Ryohei Hisano, Tatsuro
% Kawamoto, Kodai Saito, Daiki Takeuchi, Yoshitake Murai, Leo Speidel, and
% members from Imai Laboratory. In addition to the team members, I also appreciate
% people in the other teams of the project, especially, Kazuo Imai, Naonori
% Kakimura, Yusuke Kobayashi, Kohei Hayashi, Yutaro Yamaguchi, Kensuke Otsuki,
% and Satoko Tsushima.
% I also proted from several fruitful events organized by members of JST ERATO
% Minato Discrete Structure Manipulation System Project. I want to say
% thank you to people there, especially to Shin-ichi Minato, Hiroki Arimura, Koji
% Tsuda, Takeaki Uno and Yasuo Tabei.
% It was also great to be involved with Graph CREST (Advanced Computing and
% Optimization Infrastructure for Extremely Large-Scale Graphs on Post Peta-Scale
% Supercomputers). People there kindly taught me the state-of-the-art research on
% graph processing in the high performance computing community. Especially, I
% would like to thank Katsuki Fujisawa, Toyotaro Suzumura, Toshio Endo, Hitoshi
% Sato, Ken Wakita, Yuichiro Yasui and Koji Ueno.
% I also did two valuable research internships at Microsoft Research. The rst
% internship was at Microsoft Research Asia (in Beijing). I owe a big thanks to
% my mentor there, Tetsuya Sakai. I also appreciate researchers and colleagues
% there, Yuki Arase, Jun-ichi Tsujii, Mitsuo Yoshida, Jun Hatori, Hiroki Hanaoka,
% Tsuyoshi Takatani, Satoshi Ikehata, Takeshi Sakaki, Yasuhisa Yoshida, Kazuya
% Okada, Lin Meng, and Yatao Li.
% The second internship was at Microsoft Research Silicon Valley, which was
% suddenly closed in September 2014, during my internship. I would never forget
% what happened there in front of me. I express my sincere appreciation to my
% mentor there, Daniel Delling, and group members, Robert E. Tarjan, Andrew V.
% Goldberg, Edith Cohen, Renato F. Werneck, Thomas Pajor, Daniel Fleischman
% and Ilya Razenshteyn.
% Finally, I would like to express my heartfelt appreciation to my family members,
% my friends and all of those who have supported me in any aspect of graduate
% school life.
% Takuya Akiba, December 2014
% The last but definitely not the least, I would like to express my special thanks
% to my family.

==> sec/chapter_cpe_bl.tex <==
In this chapter, we aim to design algorithms that can deal with general combinatorial constraints such as paths, mactchings, and matroids.


\section{Introduction}
\subsection{Chapter Contribution}



==> sec/futurework.tex <==



==> sec/introduction_orig.tex <==
\section{Introduction}
% The world is rife with uncertainty.
% We human beings are constantly exposed to risk or ambiguous situations;
% we live with uncertainties such as daily variations in the weather or the stock market, and we are also involved in the uncertainties of fatal events such as natural disaster, climate change, or economic recession.
% In the face of uncertainty in our lives,
% we aim to take the best possible decision based on the conjecture and past experience.
% %We also make daily variations in the weather or the stock market
% %Experience always leads us how to live with uncertainty.
% % Since underestimating or misperceiving uncertainties can lead to vital mistakes or even crisis, we should be prepared for these uncertainties

\emph{Decision making under uncertainty} is common in prudent weighing of outcomes or utility. %because we human beings are constantly exposed to risk or ambiguity situations.
% With the face of uncertainty in our lives,
% we aim to take the best possible decision based on the past experience and conjecture.
Modeling of decision making under uncertainty has been analyzed in diverse research fields such as computer science, statistics, psychology, and neuroscience.


%\subsection{Sequential Decision Making under Uncertainty}


% The origin of \emph{artificial intelligence} dates back to 1950~\citep{Turing2009} with his initial question ``Can machines think?''.
% Since then, there has been a big surge of interest
% in \emph{machine learning},
% that studies how computers can achieve human or super-human level performance on various tasks,
% and its great success has made new technologies such as facial recognition system~\citep{Bartlett2005}, self-driving cars~\citep{bojarski2016end}, conversational assistants \citep{lather1991getting}, just to mention a few.
% Machine learning is a primary mechanism for extracting patterns from data,
% which is built on statistics and probability theory.
% However, there are different purposes between statistics and machine learning;
% statistics mainly focuses on understanding the past and statistical models are designed for indentifying inference, whereas machine learning puts emphasis on making predictions/decisions to the ``unknown'' in the future.





% Sequential decision making under uncertainty abounds in real-world problems ranging from game playing and robotics to resource management, packet routing, financial portfolio management, medical treatment design, and online advertisement. 
\emph{Reinforcement learning}~\citep{Bertsekas_Tsitsiklis1996, Sutton-Barto1998},
which investigates how a computer \emph{agent} can learn the best behavior from past experience by interacting with an unknown environment,
is often considered as one of the general framework for solving sequential decision making under uncertainty~\citep{mnih2015human}.
%and can capture such a variety of sequential decision making problems.
%subfield of machine learning, can capture 
%which range from 
In reinforcement learning,
an agent takes one \emph{action} based on its own \emph{policy} that maps each state of the environment to an action.
One time step later, the \emph{reward} signal corresponding to the taken action is provided from the environment (see Figure~\ref{fig:bandit}).
The goal of reinforcement learning is to learn a good policy to maximize the cumulative reward in the long run.
In reinforcement learning, an agent has to learn from samples collected by sequential interaction with the unknown environment,
and the environment does not tell explicitly what would be the best action.
This characteristic naturally leads to the following \emph{exploration-exploitation dilemma}.
The agent is required to search the space of possible decisions for potential future benefit (exploration). At the same time, she must choose the seemingly optimal decision according to the past observation (exploitation).
To understand such a trade-off between exploration and exploitation, the area of \emph{multi-armed bandit problems} (MAB), which involves only one state,
has received much attentions in the literature as the cornerstone of the stateful reinforcement learning.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{sec/figure/bandit-crop.pdf}
    \caption{An illustration of reinforcement learning, or multi-armed bandit problems.}
    \label{fig:bandit}
\end{figure}




% This is a contrast to the \emph{supervised learning} scenario, in which training examples come
% all at once explicitly containing correct answers as supervision.
% On the other hand,


The first idea of MAB appeared early in the 20th century~\citep{Thompson1933}, motivated by the medical treatment design.
The popularization of MAB as a sequential decision making model would have been realized by the seminal work of \citet{Robbins1952} and~\citet{Lai1985}.
The model of MAB is described as the following learning problem.
% an agent takes an action and observes a stochastic reward as a response at each time step.
Suppose that there are $K$ possible actions, whose utility is unknown, and each action is associated with to an unknown probability distribution.
An action is usually called an {\em arm}, 
which characterizes the decision making problem of the agent in the following stochastic game with discrete time steps. 
At each round $t=1, 2, \ldots$,
the agent must choose an arm to pull from $K$ arms.
When each arm $i$ is pulled, the agent can observe a stochastic reward sampled from an unknown probability distribution.
The most well-studied objective is to minimize the \emph{cumulative regret},
i.e.,
the total loss between the expected reward of the optimal arm and the expected reward of the arm collected by the agent~\citep{ bubeck2012,cesa2006prediction}.


Another popular objective is to identify the best arm,
i.e.,
the arm with the maximum expected reward among $K$ arms by interacting the unknown environment.
This problem,
called {\em  pure exploration} or {\em best arm identification}\footnote{In general, pure exploration is a wider concept than best arm identification, but we use these terms interchangeably in this thesis.} in the MAB,
has also received much attention recently~\citep{Even2002,Even2006,Audibert2010,Jamieson2014,Chen2015,kaufmann2016}.
In pure exploration problems, we do not care about regrets in a test phase.
In the so-called \emph{fixed confidence setting}, given a confidence level $\delta \in (0,1)$, the agent must provide the optimal action with probability at least $1-\delta$, and a learning algorithm is evaluated by its \emph{sample complexity}, which is the number of samples an algorithm requires to output the optimal arm.
In the so-called \emph{fixed budget setting}, 
the number of trials must not exceed the given budget $T$ and the agent tries to identify the optimal action.
A learning algorithm is evaluated by the \emph{probability of error}, which is the probability that an output answered by the algorithm is not the optimal action.



%
\subsection{Major Challenges and Motivation}
Despite modern developments of reinforcement learning and MAB over nearly a century,
\emph{combinatorial actions} pose a challenge to these fields.
Algorithms for reinforcement learning or bandit problems typically require an action space to be small enough to enumerate, and how to deal with combinatorially large action space has been overlooked until recently in the literature~\citep{Sugiyama2015, Lattimore+2020}.
In many real-world scenarios, indeed, our decisions are often characterized by a combinatorial and complex structure.
For example, possible actions in real-world systems may be a subset of keywords in online advertisements~\citep{Rusmevichientong2006}, assignments of tasks to workers in crowdsoucing~\citep{Zhou2014}, or channel selection in communication networks~\citep{Huang2008}.
In traditional combinatorial optimization models,
we commonly assume that the input parameters such as edge weights in a graph are exactly known and many algorithms have been developed under this assumption.
However, input parameters in the problems might not be obtained precisely in the real world, and thus they have to be learned by collecting and observing (possibly noisy) data.
To overcome this issue,
\emph{combinatorial bandit} problems, a generalization of MAB,
have been investigated recently~\citep{cesa2006prediction}.
However, much of the research still require strong feedback that reveals outcomes from individual arms
to handle computational issues,
which might not be possible in real-world applications~\citep{chenwei13,Chen+16}.


To deal with a complicated and combinatorially large action space,
decision making algorithms should be designed to avoid computational issues.
At the same time,
statistical efficiency should also be taken into consideration when designing practical algorithms for real-world applications,
which do not require strong observation or a prohibitively large number of samples.
Therefore, major challenges are summarized as follows.

\begin{itemize}
    \item [1.] \emph{Design a computationally efficient algorithm for decision making problems in combinatorially large action spaces.}
    \item [2.] \emph{Design a statistically efficient algorithm for decision making problems only from limited observation and few samples.}
\end{itemize}
To formalize these challenges,
we focus on combinatorial bandit problems with limited feedback in this thesis.
In what follows, we will describe our challenges above and motivation for studying combinatorial bandits in more detail.

\subsection{First Challenge: Decision Making with Combinatorial Actions}

Our decisions are often conducted in the combinatorial nature.
% In many application domains, possible actions have a certain combinatorial structure.
For example, each action may be a size-$k$ subset of keywords in online advertisement~\citep{Rusmevichientong2006}, an assignment between workers and tasks in crowdsourcing~\citep{LinTian2014}, or a spanning tree in communication networks~\citep{Huang2008}.
% The most common reason to study decision making algorithms with combinatorial actions is that 
\emph{Combinatorial optimization} is one of the fundamental research fields that has extensively studied in theoretical computer science and operations research~\cite{Korte2012}.
% In combinatorial optimization model,
% given a finite set of ground elements $V$,
% combinatorial constraints $\mathcal{F} \subseteq 2^V$ and an objective function $f \mid 2^V \rightarrow \mathbb{R}$,
% decision maker is asked to select a set $S \subseteq V$ such that $S$ is feasible, i.e., $S \in \mathcal{F}$, while maximizing/minimizing the objective function $f(S)$.
% In principle, it is possible to run an algorithm that evaluates $f$ for all feasible subset to find the optimal solution since the number of subsets of $V$ is finite.
% However, such an enumerating approach is not computationally efficient and prohibitive in practical scenarios, since the size of possible subsets is exponential in the size of ground elements $|V|$.
A large number of combinatorial optimization problems have been proposed
and its methological design has provided an insight on how to design a computationally efficient method  with combinatorial actions.
However, most existing models typically require the exact parameters as inputs, which are uncertain or unknown in many modern applications such as recommender systems, crowdsourcing, and online advertisement.




Over the past decade,  mathematical optimization models that are immune to data uncertainty have been studied in the field of \emph{robust optimization}~\citep{bental2009robust, Bertsimas2011}.
In the robust optimization paradigm,
uncertainty sets may often be modeled as deterministic sets such as boxes, polyhedra, or ellipsoids.
The quality of a solution is then evaluated using the realization of the uncertainty that is most unfavorable for the decision maker.
That is, robust optimization considers the worst-case scenario given uncertainty sets, and does not discuss how to design optimal sampling strategies in combinatorial action spaces to resolve the uncertainty.


%possible actions have a certain combinatorial structure in many application domains.
Combinatorial decisions
%exemplified by finding the shortest path, a routing in communication networks,
%or an assignment between workers and tasks in crowdsourcing,
often cooccur with the notion of \emph{networks} or \emph{graphs}.
Networks are ubiquitous in the real world and many complex phenomenon or systems in nature and society can be captured by networks.
A \emph{graph} $G=(V, E)$ is a mathematical representation of a network and it consists of a set of vertices $V$, and a set of edges $E$ between pair of vertices.
A \emph{weighted graph} $G=(V, E, w)$ is a graph where each edge has a numerical weight, i.e., $w \mid E \rightarrow \mathbb{R}$.
These mathematical notions are very general and intuitive, which represent a wide variety of real-world systems. Some examples include:
\begin{itemize}
    \item \emph{Technological networks}~\citep{Broder2000}: The Internet topology such as the World Wide Web and transportation networks is a graph where vertices represent web pages/routers and edges represent connection between pairs of them. The edges could be weighted by similarity between two nodes or costs for routing.
    \item \emph{Social networks}~\citep{Scott2011}: In friendship networks and co-workers networks, individuals are vertices and ties such as friendship or business relationship between people are edges.
    The edges could be weighted by the strength of connection or similarity between two users or persons.
    \item \emph{Biological networks}~\citep{Alon1866}: In protein interaction networks, vertices correspond to proteins in a cell and edges connect two proteins if both are necessary for some biological process to occur. Edge weights represent the strength of interactions among two proteins. 
\end{itemize}

With the growth of the World Wide Web and with the development of online platforms,
computational efficiency in algorithm design for decision making must be prioritized in order to handle large-sized datasets or networks.
For instance, Facebook has over 2.5 billion users in 2020\footnote{https://www.statista.com/statistics/264810/number-of-monthly-active-facebook-users-worldwide/};
YouTube also reaches over 2 billion users and more than 500 hours of content are uploaded every minute in 2020\footnote{https://www.businessofapps.com/data/youtube-statistics/}.
While many researchers in machine learning have made effort to design sophisticated methods for various types of sequential decision making problems~\citep{Sugiyama2015,Lattimore+2020},
most existing methods are hard to scale up to significantly large or combinatorial action spaces.
Indeed, most of them typically require an action space small enough to enumerate or solving complex optimization to design a good policy~\citep{Delarue+2020r}, which might be NP-hard in combinatorial settings.


% recently studied in Soare, Lazaric, and Munos~\cite{Soare2014},
% Tao, Blanco, and Zhou~\cite{Tao2018},
% and Xu, Honda, and Sugiyama~\cite{Xu2018}.
The problem of combinatorial bandits~\citep{cesa2006prediction} is a generalization of MAB, which considers combinatorial actions; a subset of underlying arms, called a \emph{super arm}, is an action in this model, while each single arm is an action in the MAB problem.
Combinatorial bandit problems with a linear reward function can be seen as a special class of \emph{linear bandit} problems.
In linear bandits,
each arm has its own feature $x \in \mathbb{R}^d$,
while in combinatorial settings,
each action can be associated with a vector $x \in \{0, 1\}^d$.
%where n is the number of single arms
%each set of arms has the feature . 
One might think that algorithms for linear bandits can deal with combinatorial action spaces.
Most linear bandit algorithms have, however, the time complexity at least proportional to the number of arms~\citep{Dani2008, yadkori11,Kwang2017}.
Therefore, a naive use of them is computationally infeasible since the number of actions $K$ is exponential.
To increase the applicability of decision making algorithms to the real world, there is a need for scalable systems that can deal with combinatorial actions.


%In mathematical optimization models, we commonly assume that the data inputs are preciselt known and ignore the influence of parameter uncertainties on the optimzality and feasibility of the modles . I t is therefore conceivable that as the data differes from the assumed nomial values, the geberated "optimal solution" may violate critical constrants and performs poorly from an objective function point of vies. These observations motivate the need for methodologies in mathematical optimization models that solve for solutions that are immune to data uncertaity.

%Combinatorial optimization [KV02] is a very important topic in applied mathematics and theoretical computer science. It can be simply stated as finding out an object from a finite collection of candidates which minimizes (or maximizes) an associated objective function. A well-known problem involving combinatorial optimization is the traveling salesman problem (TSP), which concerns finding a shortest tour that starts in a city, traverses each other city exactly once, and finally returns to the start city. Actually, combinatorial optimization can be seen almost everywhere in reality. In logistics, we may need to determine routes with a minimal total delivering cost for a fleet of vehicles which are employed to deliver goods from a central depot to consumers who ordered the goods. In a water supply system, we may need to place several valves at pipes’ extremes such that when a pipe breaks, it is possible to isolate it with minimal damage to the rest of the network. In a factory, we may need to arrange some jobs on some machines such that the resulting makespan becomes minimal. In a harbor, we may need to determine a minimal number of ships for loading certain goods which are of different volumes and shapes. In comb

%The graph is one of the most common structures in computer science,
%modeling among other things roads, communication and transportation networks, electrical circuits, relationships between individuals, corporate hierarchies, hypertext collections,
%tournaments, resource allocations, pro ject plans, database and program dependencies, and %parallel architectures.

%Combinatorial Optimization is an important area of computer science that has many theoretical and practical applications. Many real world problems in the areas of production, scheduling, resource allocation, facility location and layout, etc, can be expressed as combinatorial optimization problems. In a combinatorial optimization problem, we have a finite set of options, and we wish to find the one which is optimal with respect to some objective function, e.g., cost, time. The ability to find good or optimal solutions to real world combinatorial optimization problems can often translate into significant time, resource or monetary savings for industry.

%Combinatorial Optimization Problems are very common in industrial processes and planning activities. They are problems where a solution is composed by a set of fundamental discrete decisions or assumptions. Every decision may influence the global cost and the feseability of the solution. The trivial way to solve a combinatorial optimization problem is to enumerate the elements of the correspondent feasible solutions set and pick up the best one. But, due to the combinatorial nature of the considered problems, in real cases the number of solutions (feasible or unfeasible) to be enumerated for a given problem is intractable even for very powerful computers. To deal with the difficulty in solving Combinatorial Optimization Problems, some techniques have been proposed: • Branch and Bound methods where the solution space is systematically divided and its subsets of solutions are evaluated according to their bounds on the objective function value; • Heuristic methods, where the problem is solved through the application of experience-based techniques. When these techniques dirive from other generic or natural problems rather than the original problem, we call them Meta-heuristic; • Methods based on Integer/Mixer Programming and Hybrid methods that combine some of previously mentioned approaches.

%graph A graph consists of a pair G = (V, E) with vertices v ∈ V and edges e ∈ E ⊆ V × V . Let n represent the number of nodes, i.e. n = |V |, and m the number of edges of G, i.e. m = |E|. An edge, e, spanning two vertices, vi and vj , is denoted by eij . In this thesis, we deal with weighted graphs that include weights on both edges and nodes. An edge weight is a value assigned to each edge eij , and is denoted by wij . We assume that wij ∈ R ∗ + and use w to denote the vector of R m containing the wij for every edge eij of G. In addition to edge weights, we may also assign weights to nodes. The weight of node vi is denoted by gi . In this work, we also assume that gi ∈ R ∗ +. We use g to denote the vector of R n containing the gi for every node vi of G.





\subsection{Second Challenge: Learning with Limited Observation and Few Samples}



% Optimization under parameter uncertainty has long been
% a focus of the mathematical programming community~\cite{Bertsimas2011}
% Methodologies in  have been studied .
% To model the uncertainty of data input, robust optimization model assumes that uncertain set for the problem parameters is given.
% For example, consider a graph with uncertain edge weights.




In the stochastic combinatorial bandit framework, outcomes from super arms are assumed to follow unknown probability distributions.
In each round,
one super arm is pulled and the outcomes depending on the pulled super arm are revealed.
This learning paradigm would be a strong tool for handling combinatorial decision making with incomplete data or inaccurate measurements, and has attracted much attention~\citep{chenwei13}. Adversarial cases, in which an adversary controls the arms and tries to defeat the learning process, have also been studied in the literature~\citep{Cesa2012, Combes2015}. Adversarial cases with linear objectives have also been studied as \emph{online linear optimization}~\citep{Abernethy+2008}.



Early attempts in combiantorial bandits assume that an agent can observe the outcomes of all arms in the super arm, which is called \emph{semi-bandit} feedback~(e.g.~\citep{chenwei13, kveton15,ChenJMLR17,Zheng2017,pierre2019}).
To be more precisely, the setup of stochastic combinatorial bandits and feedback models with a linear objective are described as follows.
Let $[d]=\{1,2,\dots, d\}$ be a set of base arms.
Given combinatorial constraints,
the set of arms $\cX \subseteq \{0,1\}^d$ is a family of super arms, where each element $x \in \{0,1\}^d$ is an indicator vector of a super arm satisfying the given combinatorial structure such as a size-$k$ subset, path, or matching.
Let $X_t(e)$ for $e \in [d]$ be a random variable at round $t$ independently sampled from the associated unknown distribution.
In each round $t$, an agent selects a super arm $x_t \in \cX$ and observes some feedback. Here, the reward vector $X_t \in \mathbb{R}^d$ has its $e$-th element with $X_t(e)=\theta(e)+ \epsilon_t(e)$, where $\theta(e)$ is the expected reward and $\epsilon_t(e)$ is the zero-mean noise.
The feedback can be categorized into the following types.

\begin{itemize}
     \item [(i)]\emph{Semi-bandit feedback}: After pulling a super arm $x_t$ at round $t$, the component $X_t(e)$ for $e \in [d]$ is observed if and only if $x_t(e)=1$.
      \item [(ii)]\emph{Full-bandit feedback}: After pulling a super arm $x_t$ at round $t$, only the sum of rewards $x_t^\top X_t$ is observed.
       \item [(iii)]\emph{Partial-linear feedback}: After pulling a super arm $x_t$ at round $t$, only  $M_{x_t} \cdot X_t$ is observed, where $M_{x_t}$ is a transformation matrix $\mathbb{R}^{m_{x_t} \times d}$ whose row dimension $m_{x_t}$ depends on $x_t$. That is, the agent only observes a linear combination of rewards of $x_t$.
\end{itemize}

% $M_t^{\top}X(t)=\sum_{i=1}^n M_i X_i(t)$, where the reward $X(n) \in \mathbb{R}^d$ follows unknown probability distribution. 

% For a vector $x \in \mathbb{R}^d $ and a matrix $B\in \mathbb{R}^{d\times d}$, let $\|x\|_B=\sqrt{x^\top Bx}$. 
% For a vector $\theta \in \mathbb{R}^d$
% and a subset $S \subseteq [d]$, 
% we define $\theta(S)  =\sum_{e\in S} \theta(e)$.  
% % For clarity, we call each arm as a \textit{single-arm} and an element in decision class, which is a set of single-arms, as \textit{super arm}.
% Suppose that there are $d$ single-arms associated with unknown reward distributions $\{\phi_1,\dots, \phi_n\}$.
%semi-bansdit; phi 1 kar phi nの分布からのサンプルをそれぞれ独立に観測できる X_e
%全バンディットでは観測できない x_eの和→問題設定，
%full-saemi  / combandit linear 
%agent choose k subset; get reward;
Most prior work have studied the semi-bandit feedback~\citep{chenwei13, Chen+16}.
However, in most application domains, such strong feedback is not always available,
since it is costly to observe
a reward of individual arms, 
or sometimes we cannot access feedback from individual arms.
% For example,
% in cognitive ratio networks,
% we wish to allocate multiple channels
% with efficiency~\cite{Huang2008},
% but evaluating each communication cost of each channel 
For example, in crowdsourcing,
we often obtain a lot of labels given by crowdworkers,
but it is costly to compile labels according to labelers.
In the case of transportation networks, it is not easy to observe a delay of each section of a path due to some system constraints.
%Moreover, labeling tasks may include difficult ones that require some specialized knowledge.
In social networks, due to some privacy concerns and data usage agreements, 
it may be impossible even for data owners to obtain the estimated number of messages exchanged by two specific users.
To overcome these issues, algorithms that can deal with full-bandit feedback or partial-linear feedback are desired.
However, there are very few studies even for the full-bandit feedback in the combinatorual bandit literature~\citep{TalebiMazraehShahi2016}.
%~\citep{agrawal2000privacy,zheleva2011privacy}.

% The agent chooses a size-$k$ subset
% from $d$ single-arms at each round $t$ for an integer $k>0$.
% In the well-studied {\em semi-bandit} setting,
% the agent pulls a subset $M_t$,
% and then she can observe $X_t(e)$ for each $e \in M_t$ independently sampled from the associated unknown distribution $\phi_e$.
% %The sum of rewards $r_{M_t}$ for a size-$k$ subset $M_t$ is expressed by $r_{M_t}= \theta(M_t)+\sum_{e \in M_t}\epsilon_t(e)$.
% However, in the {\em full-bandit} setting,
% she can only observe the sum of rewards $r_{M_t}= \theta(M_t)+\sum_{e \in M_t}\epsilon_t(e)$ at each pull,
% which means that
% estimators of expected rewards of single-arms are no longer independent of each other.
% % MP-MAB has received much attention and several algorithms have been proposed for regret minimization~\citep{agrawal1990multi,anantharam1987,  Komiyama2015,largre2016}.

Why is dealing with such limited feedback hard?
Stochastic bandit problems have been analyzed by two different approaches:
a frequentist approach, where the parameter is a deterministic unknown quantity, and a Bayesian approach, where the parameter is drawn from a prior distribution.
Vast majority of combinatorial and linear bandit work follow a frequentist approach.
They often employ the optimism principle examplified by \emph{upper confidence bound} (UCB) algorithm~\citep{yadkori11,Chen+16}, which uses the data observed so far to assign to each arm a value, called the UCB that is an overestimate of the unknown mean with high probability.


To handle full-bandit feedback, the frequentist approach may rely on the least-square estimator, and the combinatorial structure results in a confidence region in the form of an ellipsoid.
With a confidence ellipsoid, algorithms often require complex optimization for determining the next arm to pull, which might involve quadratic optimization with combinatorial constraints. All the existing linear bandit algorithms execute a brute-force search to solve such an optimization problem and thus they cannot be naively applied to combinatorial bandit problems. Therefore, we need to develop different techniques to deal with  full-bandit feedback in combiantorial settings.

The model of partial-linear feedback addresses general limited feedback that ranges from semi-bandit to full-bandit feedback. 
For regret minimization,
several researchers investigated UCB-based algorithms~\citep{LinTian2014,Sougata-Ambuj2016}.
On the other hand, for the pure exploration problems, there is no existing study and it has been open to investigate which combinatorial problems are still polynomial-time learnable.


For regret minimization, many algorithms in various settings are already shown to achieve sublinear regret bounds in time horizon $T$ and the achievable theoretical limit is becoming now well known.
On the other hand,
much remains to be done for the pure exploration problems~\citep{kaufmann2016}.
The pure exploration problem models situations in which costs are not measured in terms of rewards but rather in terms of resources~\citep{Bubeck2011}.
Since we aim to design statistically efficient algorithms that require less samples while guaranteeing that the output is optimal in the pure exploration problem,
good algorithms for pure exploration would require quite different strategies from those for regret minimization.
It is important to care about the dependence of the minimum gap $\Delta_{\min}$, i.e., the reward gap between the best action and the second best one;
this quantity is crucial in the sample complexity analysis for pure exploration problems.
In many practical applications,
$\Delta_{\min}$ is often too small~\citep{Kawase+19}, and heavy dependence on $1/\Delta_{\min}$ means that a large number of samples are required to identify the optimal action.
Therefore, we wish to develop algorithms whose sample complexity only has mild dependence on $1/\Delta_{\min}$.




% Bubeck et al. (2011) show that in the fixed-budget setting, when m = 1, any sampling
% strategy designed to minimize regret performs poorly with respect to the simple regret
% rt
% := µ
% ∗ − µSˆ1
% , which is closely related to the probability pt(ν) of recommending the wrong
% arm. Therefore, good strategies for best-arm identification need to be quite different from
% regret-minimizing strategies.

%  I t is therefore conceivable that as the data differes from the assumed nomial values, the geberated "optimal solution" may violate critical constrants and performs poorly from an objective function point of vies. These observations motivate the need for methodologies in mathematical optimization models that solve for solutions that are immune to data uncertaity.
% In many real-world scenarios, indeed, our decisions are often characterized by a combinatorial and complex structure.
% For example, possible actions in real-world systems may be a subset of keywords in online advertisements, assignments of tasks to workers in crowdsoucing, or paths in communication networks.




% \paragraph{Robust Optimization.}

% \paragraph{Combinatorial Bandits.}

%普通の組合せ最適化では不確実性やオンラインでデータを集めることは考えられていない Massive datasets abound. For instance, Google has been processing more than 20 Petabytes of data on a day-to-day basis for nearly a decade now [115], Facebook graph has contained more than trillion edges for quite some time [100], and in some applications, we now need to process streams of data at a rate of Gigabytes per second [91]. The need to process such massive datasets necessitates rethinking the task of algorithm design as the traditional computational models do not capture these scenarios accurately. For instance, it is no longer realistic to assume the standard random access model where the data can be accessed in an arbitrary order and that each data access has unit cost. As a result, we are now encountering a paradigm shift toward modern computational models that can more accurately capture the essence of computation on massive datasets.

%write combinatorial bandit$
% write feedback model bandit, semi-bandit, partial bandit 


\section{Thesis Statement and Contributions}

In this thesis, 
we study several stochastic combinatorial bandit problems on the pure exploration settings.
This thesis provides evidence to support the following statement:
\vspace{1cm}
  \begin{itembox}{Thesis Statement}
\emph{One can efficiently solve combinatorial decision making problems even when input parameters are initially unknown and only limited observation is available.}
  \end{itembox}
\vspace{1cm}
% is thesis gives evidence to support the following statement:
% Ecient combinatorial optimization is possible even when the underlying input is uncertain
% and we (adaptively) make irrevocable decisions to resolve this uncertainty.

%time complexity and quality of solution + sample complexity
% In this Thesis, we present a new class of nonmyopic approaches for solving complex sensing problems.
% We claim the following statement:
% In many practical applications, it is important to select among useful but expensive
% observations. By exploiting problem structure, one can efficiently and near-optimally
% solve many of the resulting sensing problems.

We believe that the results developed in this thesis will motivate future researchers in both optimization and bandit communities to develop algorithms for combinatorial decision making under uncertainty.
In order to substantiate this statement, we present the following contributions.
%The summary of theoretical results can be found in Table~\ref{table:summary_results}.

% \begin{table*}[t]
% 	\centering
% 	\caption{Comparison between our results and state-of-the-art results for CPE-BL(PL). ``General'' represents that the algorithm works for any combinatorial structure. $\tilde{O}(\cdot)$ only omits $\log \log$ factors. Main notations are defined 
% %	A full table and specific notations are given in Appendix~\ref{apx:related_work}. 
% 	} 
% 	\label{table:summary_results}
% 	\scalebox{0.55}{
% 	\begin{tabular}{|c|c|c|c|c|c|}
% 		\hline
% 		Authors&Fixed Confidence/Budget&Case&Problem Type&Strategy&Time\\
% 		\hline
		
% 		 Chapter~\ref{chap:pre} &$\tilde{O}\big(\frac{d^{1/4}k\xi_{\max}({M({\lambda})}^{-1})\rho(\lambda)}{\Delta_{\min}^2} \log \frac{d^{1/4}k\xi_{\max}({M({\lambda})}^{-1})\rho(\lambda)}{\Delta_{\min}^2  \delta}\big)$ &Top-$k$ &CPE-BL& Static&$\mathrm{Poly}(d)$ \\
% 		\hline		 
% 		{\bf 
% 		\textsf{GCB-PE} (ours, Thm.~\ref{thm:GCB_ub})} &$O \big( \frac{ |\sigma| \beta_{\sigma}^2 L_p^2}{\Delta_{\textup{min}}^2} \log \frac{ \beta_{\sigma}^2 L_p^2}{\Delta_{\textup{min}}^2\delta} \big)$& General &CPE-PL&Static&$\mathrm{Poly}(d)$\\
% 		\hline
% 		{\bf  
% 		\textsf{PolyALBA} (ours, Thm.~\ref{thm:CPE-BL})} &$\tilde{O} \big(\sum_{i=2}^{\lfloor \frac{d}{2} \rfloor} \frac{1}{\Delta_i^2} \log \frac{|\mathcal{X}|}{\delta}    +\frac{d^2 m \xi_{\max}({\widetilde{M}({\lambda})}^{-1})}{ \Delta^2_{d+1}} \log \frac{|\mathcal{X}|}{\delta} \big)$&General &CPE-BL& Adaptive  &$\mathrm{Poly}(d)$\\
% 		\hline
% 		\textsf{CSAR}~\cite{Idan2019} &$\tilde{O}\big(\sum^{d}_{i=2}\frac{1}{\tilde{\Delta}_i^2} \log\frac{d}{\delta}\big)$&Top-$k$ &CPE-BL&  Adaptive &$\mathrm{Poly}(d)$ \\
% 		\hline
% %		\textsf{$\mathcal{X}\mathcal{Y}$-static}~\cite{Soare2014}&$O\big(\frac{d}{\Delta_{\textup{min}}^2}\log \frac{|\cX|}{\delta \Delta^2_{\min}} +d^2\big)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Static& $\Omega(|\cX|)$ \\
% %		\hline
% %		\textsf{\textsf{Explore-Verify}}~\cite{Karin16}&$O\big(\frac{d}{\Delta_{\textup{min}}^2} \log \frac{|\cX|}{\delta \Delta_{\min}}+ d\log \delta^{-1}\big)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Static& $\Omega(|\cX|)$\\
% %		\hline
% %		\textsf{LinGapE}~\cite{Xu2018}&  $\tilde{O}\big(d  \sum_{x \in \cX} H_x\log \frac{d|\cX|}{\delta} \cdot \sum_{x \in \cX} H_x\big)$ &$\cX \subseteq \mathbb{R}^d$&BAI-LB& Adaptive & $\Omega(|\cX|)$\\
% %		\hline
% %		$\mathcal{Y}$-\textsf{ElimTil}~\cite{Tao2018}&$\tilde{O}\big(\frac{d}{\Delta_{\textup{min}}^2} (\log \delta^{-1} + \log |\mathcal{X}|)\big)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Adaptive& $\Omega(|\cX|)$\\
% %		\hline
% 	    \textsf{ALBA}~\cite{Tao2018}&$\tilde{O}\big(\sum^{d}_{i=2}\frac{1}{\Delta_i^2}(\log \delta^{-1} + \log |\mathcal{X}|)\big)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Adaptive & $\Omega(|\cX|)$\\
% 		\hline
% 		\textsf{RAGE}~\cite{Fiez2019}&$O \big(\sum^{\left \lfloor \log_2(4/\Delta_{\min})  \right \rfloor}_{t=1} 2(2^t)^2\tilde{\rho}(\mathcal{Y}(S_t)) \log(t^2|\mathcal{X}|^2/\delta) \big)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Adaptive& $\Omega(|\cX|)$\\
% 		\hline
% 		\textsf{LinGame(-C)} \cite{Degenne+2020}&$\mathop{\lim \sup}_{\delta \rightarrow 0} \frac{\mathbb{E}_{\theta}[\tau_{\delta}]}{\log(1/ \delta)} \leq \min_{\lambda \in \triangle(\cX)}\max_{x\in \mathcal{\cX} \setminus\{x^*\}} \frac{2||x^*-x||_{M(\lambda)^{-1}}^2}{((x^*-x)^{\top}\theta)^2} $&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Adaptive& $\Omega(|\cX|)$ \\
% 		\hline
% 		\textsf{Peace} \cite{Katz+2020}&$O\big( (\min_{\lambda \in \triangle(\cX)}\max_{x\in \mathcal{\cX} \setminus\{x^*\}} \frac{||x^*-x||_{M(\lambda)^{-1}}^2}{((x^*-x)^{\top}\theta)^2} + \gamma^* )  \log(1/ \delta)\big)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Adaptive& $\Omega(|\cX|)$ \\
% 		\hline
% 		Lower Bound \cite{Fiez2019}&$\mathbb{E}_{\theta}[\tau_{\delta}] \geq \min_{\lambda \in \triangle(\cX)}\max_{x\in \mathcal{\cX} \setminus\{x^*\}} \frac{||x^*-x||_{M(\lambda)^{-1}}^2}{((x^*-x)^{\top}\theta)^2} \log(1/2.4 \delta)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& - & - \\
% 		\hline
% 	\end{tabular}
% 	}
% \end{table*}

\subsection*{Chapter~\ref{chap:topk}: Top-$k$ Arm Identification with Full-bandit Feedback}

\paragraph{Problem and Motivation.}
We start with the simplest case in terms of combinatorial structures.
We study the problem of stochastic {\em top-$k$ arm identification}, where an agent sequentially explores a size-$k$ subset of arms (super arm) from given $d$ arms and tries to identify the best super arm. 
The problem is also called the {\em  top-$k$ selection}
or {\em $k$-best arm identification},
and there is an emerging body of work in the bandit literature~\citep{bubeck2013, Cao2015,  Gabillon2011,Gabillon2012,kalyanakrishnan2010,kalyanakrishnan2012, kaufmann2013, Roy2017, Roy2019, Zhou2014}.
In the above prior work, we need a strong assumption that the agent is allowed to pull a base arm and can observe its outcome directly at all rounds, which might not be possible in real-world scenarios.
Our study is the very first work to analyze the top-$k$ arm identification with full-bandit feedback, and we find a variety of applications for full-bandit settings. Some application examples are:
\begin{itemize}
    \item \emph{Online advertisement auctions:} Companies may want to choose multiple keywords to promote their products to consumers based on their search queries.
From millions of available choices,
a company aims to find the most effective set of keywords by observing the historical performance of the chosen keywords.
In such application domains, we may be interested in best-$k$ keywords and only the total sum of clicks can be sequentially observed.
This decision making problem is formulated as top-$k$ arm identification with full-bandit feedback,
where each arm corresponds to each keyword and reward corresponds to the effectiveness or utility of a keyword. 
    \item \emph{Extracting experts in crowdsourcing:} A system-owner or employer may often obtain a lot of labels given by crowdworkers,
but it is costly to compile labels according to labelers.
%Moreover, labeling tasks may include difficult ones that require some specialized knowledge.
Furthermore,
in software projects,
an employer may have complicated tasks that need multiple workers, in which the employer can only evaluate the quality of a completed task rather than the performance of a single worker.
In such scenarios,
we wish to extract top-$k$ expert workers who can perform the task with high quality, 
only from a sequential access to the quality of the task completed by multiple workers.
\end{itemize}

\paragraph{Contribution.}
Although our problem can be regarded as an instance of the best arm identification problem in linear bandits, a naive approach based on linear bandits is computationally infeasible since the number of super arms $K$ is exponential.
We first show that quadratic optimization with the size constraint involved in existing linear bandit algorithms is naturally stated as a uniform knapsack problem, which is NP-hard.
To cope with this computational issue, we first design a polynomial-time approximation algorithm for a 0-1 quadratic programming problem to obtain the maximum width of a confidence ellipsoid.
Based on our approximation algorithm,
we propose the first bandit algorithms, namely {\tt SAQM}, that runs in $O(\log K)$ time
and provide an upper bound of the sample complexity,
which is still worst-case optimal.
The result indicates that our algorithm provides an exponential speedup over an exhaustive search algorithm while keeping the statistical efficiency.
We also design two heuristic algorithms that empirically perform well:
{\tt SA-FOA} using first-order approximation 
and {\tt CLUCB-QM} based on the lower-upper confidence bound algorithm.
%that empirically perform well.
Finally,
we conduct experiments on synthetic and real-world datasets with more than $10^{10}$ super arms, demonstrating the superiority of our algorithms in terms of both the computation time and the sample complexity.

% This chapter is based on a paper with Liyuan Xu, Atsushi Miyauchi, Junya Honda and Masashi Sugiyama~\citep{Kuroki+19} in Neural Computation.
%  \chapter{Combinatorial Pure Exploration with Full-bandit Feedback}\label{chap:CPE-BL}
% \chapter{Online Dense Subgraph Discovery via Linear Feedback}\label{chap:dense}
% %   \input{ICML2020/icml_main}
%  \chapter{Combinatorial Pure Exploration with partial-linear Feedback}\label{chap:CPE-PL}

\subsection*{Chapter~\ref{chap:CPE-BL}: Combinatorial Pure Exploration with Full-bandit Feedback under General Constraints}



\paragraph{Problem and Motivation.}
How can we go beyond the top-$k$ setting in the full-bandit setup?
 We next seek how to deal with more complex combinatorial constraints such as paths, spanning trees, and matchings.
In the offline settings,
such structures are very common and fundamental combinatorial optimization problems such as the shortest path, the minimum spanning tree, and the weighted matching problems have been extensively studied in theoretical computer science (definitions of these problems will be introduced below).
For the top-$k$ case in the bandit setting, we find that there exists a naive reduction to the classical combinatorial pure exploration problem, in which the agent directly samples a base arm at each round. 
However,
for more complex cases such as matroids, matchings,
and $s$-$t$ paths,
we cannot use such a reduction due to their combinatorial constraints.
To increase the applicability of bandit methods,
we propose a novel algorithm for \emph{combinatorial pure exploration with full-bandit linear feedback (CPE-BL)}, where underlying combinatorial structures are matroids, matchings, and $s$-$t$ paths and the reward function is a linear objective.
Some examples of offline combinatorial problems in CPE-BL are as follows.
%and its uncertainty on input parameters are described as follows:

\begin{itemize}
    \item The \emph{shortest path problem:} Given a directed graph $G=(V, E)$ and a cost (or time length) $\theta_e$ assigned to each edge $e \in E$,
the shortest path problem is to find the path $P$ from origin node $s$ to destination node $t$ that minimizes the sum of costs $\sum_{e\in P}\theta_e$.



    \item The \emph{minimum spanning tree problem:} A spanning tree on a graph is a set of edges
which connects all the vertices. Given an undirected graph $G=(V, E)$ with a cost $\theta_e$ assigned to each edge $e \in E$,
    the minimum spanning tree problem is to find the spanning tree $T$ that minimizes the sum of costs $\sum_{e\in T}\theta_e$.
    \item \emph{The weighted matching problems:} A matching on a graph is a set of vertex-disjoint edges. Suppose that we are given an undirected graph $G=(V, E)$ with a weight $\theta_e$ assigned to each edge $e \in E$. The \emph{minimum cost matching} problem is to find the matching that minimizes the sum of costs $\sum_{e\in P}\theta_e$.
    The \emph{maximum weight matching problem} is to find the matching that maximizes the sum of weights $\sum_{e\in P}\theta_e$. A special case of the problem is the \emph{assignment problem}, in which the given graph is a bipartite graph.

    
\end{itemize}
These combinatorial optimization problems are very fundamental and have a rich history,
and several polynomial-time algorithms are known to these problems~\citep{dijkstra1959note,edmonds_1965, Korte2012}.
In real-world scenarios, however,
input parameters such as the cost $\theta_e$ for each $e \in E$ of the combinatorial problems above are often unknown and have uncertainty.
Our learning model of CPE-BL can capture these situations,
in which a base arm corresponds to an edge, and rewards correspond to costs.
For example, in the case of communication networks, a decision maker may not get access to the exact information of transmission delay for each arc. 
In this scenario, decision maker sequentially selects a routing that forms required structures such as a path, spanning tree, or matching in communication networks.
Then the decision maker tries to identify the best routing as soon as possible only with a sequential access to the total cost for the chosen routing (see Figure~\ref{fig:examples} for application examples). 

A \emph{static} algorithm, which samples super arms based on the predetermined arm-selection ratio without any observation, might be useful for reducing computational costs.
However, such a static sampling strategy may degrade the sample complexity and result in heavy dependence on the minimal gap.
On the other hand, an \emph{adaptive} algorithm,
which changes sampling strategies based on past observations,
may require more complex minimax optimization, which is intractable in the combinatorial action space.

\begin{figure}
    \centering
    \subfigure[A spanning tree in communication networks]{\label{fig:spanningtree}
    \includegraphics[width=0.32\textwidth]{sec/figure/communication_network-crop.pdf}
    }
    \hspace{1.5cm}
    \subfigure[An assignment in wireless networks]{\label{fig:matching_BL}
        \includegraphics[width=0.45\textwidth]{sec/figure/wirelessnetwork-crop.pdf}
        }
    \caption{The examples of combinatorial structures in networks.}
    \label{fig:examples}
\end{figure}


\paragraph{Contribution.}

We begin with a discussion on a fully-adaptive algorithm for CPE-BL and the result depends on a non-controllable term (i.e., the minimum eigenvalue of the information matrix), indicating that fully-adaptive control among all super arms may be difficult.
As a remedy for these issues, we propose an algorithm, namely \textsf{PolyALBA}, in which we have two phases: the first phase is for finding a polynomial-size set of super arms which contains the optimal super arm with high probability and discards other super arms. The second phase focuses on sampling super arms among the rest by adaptive elimination procedures. 
To the best of our knowledge,
our \textsf{PolyALBA} is the first adaptive and polynomial-time algorithm that works for general combinatorial structures and avoids heavy dependence on the minimum gap.
We show that the sample complexity of \textsf{PolyALBA} matches (within a logarithmic factor) the information theoretic lower bound for a family of instances.
 We conduct a series of experiments for CPE-BL on the matching and top-$k$ instances. The experimental results demonstrate that (a) \textsf{PolyALBA} scales to  combinatorial instances while existing linear bandit algorithms require prohibitive amount of time;
 (b) the number of samples required by \textsf{PolyALBA} is not sensitive to the value of the minimum gap.

% This chapter and Chapter~\ref{chap:CPE-PL} are based on a working paper with Yihan Du and Wei Chen.



\subsection*{Chapter~\ref{chap:dense}: Online Dense Subgraph Discovery via Linear Feedback}


\paragraph{Problem and Motivation.}
What if the reward function is no longer linear in combinatorial pure exploration problems? Can we utilize the property of graph structures to resolve non-linearity? We study a bandit model of the \emph{densest subgraph problem}, one of the most fundamental graph optimization problems with nonlinear objective functions, as a cornerstone to investigate these questions.

\emph{Dense subgraph discovery} aims to find a dense component in edge-weighted graphs and this is a fundamental task for graph mining with a variety of applications~\citep{Dourisboure+07,Gibson+05,Bader_Hogue_03,Kawase+19,Angel+12} (see Figure~\ref{fig:graphmining}).
In the densest subgraph problem, given an edge-weighted undirected graph, we are asked to find a subset of vertices that maximizes the so-called \emph{degree density}, which is defined as half the average degree of the subgraph induced by the subset. 

Whereas most existing algorithms for the densest subgraph problem require a full input of the graph data, in many real-world applications, the edge weights need to be estimated from {\em uncertain} measurements.
A measurement for individual edges is often quite costly or sometimes impossible due to privacy concerns or system constraints.
On the other hand, it is often affordable to observe aggregated information of a subset of edges,
because this procedure reveals much less information of individual users or requires less cost to conduct~\citep{agrawal2000privacy,zheleva2011privacy}.
For such dense subgraph discovery under uncertainty, we introduce a novel learning problem
by incorporating the concepts of stochastic combinatorial bandits into the densest subgraph problem.
In this problem, an agent is given an undirected graph, whose edge weights are associated with unknown probability distributions.
During the exploration period,
the agent chooses a subset of edges (rather than a single edge) to sample,
and observes the sum of noisy edge weights in the queried subset.
After the exploration period is over,
the agent must report one subgraph that she believes to be optimal.


\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{sec/figure/graphmining-crop.pdf}
    \caption{The process of dense subgraph discovery.}
    \label{fig:graphmining}
\end{figure}

\paragraph{Contribution.}
We study the both fixed confidence and fixed budget settings.
For the former setting, we present an algorithm \textsf{DS-Lin}; for its design, we follow techniques of pure exploration in linear bandits and provide a sample complexity bound, which is the first polynomial-time sample complexity result for this problem.
Our key idea is to utilize an approximation algorithm for unconstrained quadratic optimization to compute the maximal confidence bound,
%using semidefinite programming,
thereby guaranteeing that the output by \textsf{DS-Lin} is an $\epsilon$-optimal solution and the running time is polynomial in the size of a given graph.
For the fixed budget setting,
we design a scalable and parameter-free algorithm \textsf{DS-SR} that runs in $O(|V|^2 T)$ time complexity for the given budget $T$, while \textsf{DS-Lin} needs $O(|E|^2)$ time for updating the estimate.
%, where $d$ is the size of vertices.
Our key idea is to combine the {\em successive reject} strategy~\citep{Audibert2010} for the multi-armed bandits and the {\em greedy peeling} algorithm~\citep{Charikar2000} for the densest subgraph problem.
We prove an upper bound on the probability that
\textsf{DS-SR} outputs a solution whose degree density is less than $\frac{1}{2}{\rm OPT}-\epsilon$, where ${\rm OPT}$ is the optimal value.
In a series of experiments, we thoroughly evaluate the performance of our proposed algorithms using well-known real-world graphs. 
We confirm that 
\textsf{DS-Lin} obtains a nearly-optimal solution even if the minimum size of queryable subsets is larger than the size of an optimal subset,
which is consistent with the theoretical analysis.
In the fixed budget setting, we implement a robust optimization algorithm by~\citet{Miyauchi_Takeda_18} as a baseline and observe that it requires a large number of samples for single edges. We demonstrate that \textsf{DS-SR} finds nearly-optimal solutions even for large-sized instances,
while significantly reducing the number of samples for single edges.


% This chapter is based on a paper with Atsushi Miyauchi, Junya Honda and Masashi Sugiyama~\citep{Kuroki2020} in ICML'20.

\subsection*{Chapter~\ref{chap:CPE-PL}: Combinatorial Pure Exploration with Partial-Linear Feedback for Nonlinear Rewards}
\paragraph{Problem and Motivation.}
Although full-bandit settings can capture many practical situations as demonstrated in Chapters~\ref{chap:topk}--\ref{chap:dense},
it may happen that we cannot always observe outcomes from some of the chosen arms due to privacy concern or system constraints.
To overcome this issue,
we propose a general model of \emph{combinatorial pure exploration with partial-monitoring linear feedback} (CPE-PL), which simultaneously models limited feedback, general (possibly nonlinear) reward and combinatorial action space.
The model subsumes our previous problems addressed in Chapters~\ref{chap:topk}--\ref{chap:dense}.
In CPE-PL, given a combinatorial action space $\cX \subseteq \{0,1\}^d$, where each dimension corresponds to a base arm and each action $x\in \cX$ is an indicator vector of a super arm.
In each round the agent chooses an action (super arm) $x_t \in \cX$ to pull and observes a random partial-linear feedback with expectation of $M_{x_t} \theta$, where $M_{x_t}$ is a transformation matrix for $x_t$ and $\theta \in \mathbb{R}^d$ is an unknown environment vector. 
%The agent also gains a random (possibly nonlinear) reward related to $x_t$ and $\theta$, which may not be part of the  feedback and thus may not be directly observed.
CPE-PL framework includes CPE-BL as its important subproblem;
 in CPE-BL, the agent observes full-bandit feedback (i.e. $M_x = x^{\top}$) and gains linear reward (with expectation of 
$x^{\top} \theta$) after each play. 
The model of CPE-PL appears in many practical scenarios, including:
%\begin{spacing}{0.94}
\begin{itemize}
 % \setlength{\leftskip}{-0.5cm}
%   \setlength{\itemsep}{-0.0mm} % 項目の隙間
%   \setlength{\parskip}{-0.0mm} % 段落の隙間
    \item \emph{Learning to rank.} Suppose that a company (agent) wishes to recommend their products to users by presenting the ranked list of items. Collecting a large amount of data on the relevance of all items might be infeasible, but the relevance of a small subset of items which are highly-ranked (or top-ranked item) is reasonable to obtain~\citep{Sougara-Ambuj2015,Sougata-Ambuj2016, Sougata-Ambuj2017}.
    In this scenario, the agent selects a ranked list of entire items at each step, and observes random partial-linear feedback on the relevance of highly-ranked $d' \ll d$ items. The objective is to identify the best ranking of their whole items with as few samples as possible.

    \item \emph{Task assignment in crowdsourcing.}
    Suppose that an employer wishes to assign crowdworkers to tasks with high quality performance. It might be costly for the employer and workers to provide task performance feedback for all tasks~\citep{LinTian2014}, and privacy issues may also arise.
    In this scenario, the agent sequentially chooses an assignment of workers to tasks and observes random partial-linear feedback on a small subset of completed tasks.
    The objective is to find the matching between workers and tasks with the highest performance using as few samples as possible.
    
\end{itemize}
\paragraph{Contribution.}
We focus on the fixed confidence setting and propose the first polynomial-time algorithmic framework for the general CPE-PL problem with novel sample complexity analysis. 
As an important assumption, we analyze nonlinear reward functions that satisfy Lipschitz continuity. We also assume that there exists a \emph{global observer set} $\sigma=\{x_1, x_2, \dots, x_{|\sigma|}\} \subseteq \cX$,  such that the stacked $\sum_{i=1}^{|\sigma|} m_{x_i}$-by-$d$ transformation matrix $M_{\sigma}=(M_{x_1}; M_{x_2}; \cdots; M_{x_{|\sigma|}})$ is of full column rank, i.e., $\mathrm{rank}(M_{\sigma})=d$. 
Our proposed algorithm, namely \textsf{GCB-PE},
samples each super arm in the global observer set to estimate the environment vector $\theta$ and constructs a global confidence bound, which is a confidence bound for the global observer set rather than one super arm.
Owing to a global confidence bound and Lipschitz continuity of the expected reward function,
we can determine whether the empirical best super arm is indeed the best super arm with confidence $1-\delta$ or not by simply seeing a large enough gap between the empirical best and second best super arms.
The experimental results show that our algorithm is superior in terms of speed over the existing ones, and demonstrate that \textsf{GCB-PE} is the first algorithm which can simultaneously deal with combiantorial action space, partial feedback, and nonlinear reward functions.


% \subsection{Overview of Contributions}

% Motivated by real-world applications, we develop theory and algorithms for challenging settings, in which only limited feedback is given to a agent.
% In the combinatorial bandit literature, a large amount of work has studied the \emph{semi-bandit} setting, in which a agent can directly observe a random feedback from an individual arm at each sampling trial.
% However, such a sampling procedure for individual arms is costly or often impossible due to the privacy issues or system constraints.
% To overcome this critical limitation of existing studies,
% we aim to propose statistically and computationally efficient methods based on only limited observation. To this end, we design several approximation algorithms for NP-hard problems and bandit algorithms that can deal with an aggregated feedback from a subset of arms.

\section{Thesis Organization}

\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{sec/figure/chapters-crop.pdf}
    \caption{The roadmap of this thesis.}
    \label{fig:roadmap}
\end{figure}

The organization of this thesis is summarized as follows.
In Chapter~\ref{chap:pre}, we briefly review some relevant materials on combinatorial pure exploration and necessary concept from combinatorial optimization. In Chapter~\ref{chap:topk}, we start with top-$k$ arm identifications with full-bandit feedback, the simplest case of combinatorial pure exploration with full-bandit feedback.
In Chapter~\ref{chap:CPE-BL}, we address a combinatorial pure exploration under general constraints such as paths, matchings, and matroids.
In Chapter~\ref{chap:dense}, we study a pure exploration bandit model of the densest subgraph problem, one of the most fundamental graph optimization problems with nonlinear objective functions. 
In Chapter~\ref{chap:CPE-PL}, we study a novel model of combinatorial pure exploration with partial-liner feedback, of which our models in Chapters~\ref{chap:topk}--\ref{chap:dense} are special cases.
The main technical contributions of this thesis lie in Chapters~\ref{chap:topk}--\ref{chap:CPE-PL} where efficient algorithms and theoretical results are provided for individual topics.
% In each chapter, we begin with an introduction and related work on the topic, and then state the formal problem definition. Next we present the main methodological contributions and provide theoretical analysis. Finally we present empirical results.
Chapter~\ref{chap:conclusion} concludes with the summary of this thesis and discussion on future work. The roadmap of this thesis can be found in Figure~\ref{fig:roadmap}.



% \section{Machine Learning}
% \subsection{Reinforcement Learning}



==> sec/last_chapter.tex <==
 In this chapter, we conclude the thesis. Specifically, we summarize the contribution of the thesis and discuss future directions.
 
 \section{Summary}
 
This thesis has been devoted to investigating the learnability of the stochastic combinatorial pure exploration problems with limited feedback.
Our main goal was to develop polynomial-time algorithms for such combinatorial pure exploration problems with theoretical guarantee, while most of the existing algorithms require the exponential time (e.g.~\citep{Soare2014,Karin16,Xu2018,Tao2018,Fiez2019,Degenne+2020,Katz+2020}) or strong feedback ( e.g.~\citep{bubeck2013, Cao2015,  Gabillon2012,Gabillon2011,kalyanakrishnan2010,kalyanakrishnan2012, kaufmann2013, Roy2017, Roy2019, Zhou2014,Cao2019, Chen2014,Chen2016matroid, Chen17a,Gabillon2016}).
Our results provide novel insights into how to solve online decision making problems  in combinatorial action spaces only with limited observation.


In Chapter~\ref{chap:topk},
the problem of top-$k$ arm identification with full-bandit feedback has been discussed.
% we designed a novel approximation algorithm
% for 0-1 quadratic maximization with theoretical guarantee. 
% Based on our approximation algorithm,
% we proposed polynomial-time algorithms {\tt SAQM} and {\tt SA-FOA} and provided the upper bound of the sample complexity,
% which matches the worst-case optimal.
% Finally,
% we conducted experiments on synthetic and real-world datasets with more than $10^{10}$ super arms.
% There are several directions for future research.
% It remains open to design adaptive algorithms with problem-dependent optimal sample complexity. It is also interesting question about the lower bound of any $(\epsilon, \delta)$-PAC algorithm that works in polynomial-time.
%%%%%%%%%%%%%%%%%%%%%%%%%%long ver%%%%%%%%%%%
We have designed a novel approximation algorithm with theoretical guarantee
for a 0-1 quadratic programming problem arising in confidence ellipsoid maximization. 
Based on our approximation algorithm,
we have proposed the $(\epsilon, \delta)$-probably approximately correct (PAC) algorithms {\tt SAQM} that run in $O(\log K)$ time
and provided an upper bound of the sample complexity,
which is still worst-case optimal;
the result indicates that our algorithm provided an exponential speedup over exhaustive search algorithms while keeping the statistical efficiency.
We have also designed two heuristic algorithms that empirically perform well:
{\tt SA-FOA} using first-order approximation 
and {\tt CLUCB-QM} based on lower-upper confidence bound algorithm.
%that empirically perform well.
Experimental results have demonstrated the superiority of our algorithms in terms of both the computation time and the sample complexity.
%There are several directions for future research.


% It remains open to design adaptive algorithms with a problem-dependent optimal sample complexity. It is also interesting question to seek a lower bound of any $(\epsilon, \delta)$-PAC algorithm that works in polynomial time. Extension for combinatorial pure exploration under general constraints with full-bandit feedback is another direction.



In Chapter~\ref{chap:CPE-BL},
the problem of combinatorial pure exploration with full-bandit feedback (CPE-BL) has been discussed.
% We design the first polynomial-time adaptive algorithm \textsf{PolyALBA} for CPE-BL, propose the general CPE-PL framework and provide the first polynomial-time algorithm \textsf{GCB-PE} for CPE-PL.
%	
%
%
%
%
%problem, in which a learner pulls an action from a combinatorial space and receives a full-bandit random reward at each timestep, with the objective of identifying the optimal action. 
We have designed the first adaptive algorithm \textsf{PolyALBA} that runs in polynomial time with the aid of G-optimal design. 
We have shown that the sample complexity of \textsf{PolyALBA} achieves the worst-case optimality for a family of instances.
The proposed method empirically performed better than a static algorithm proposed in Chapter~\ref{chap:topk} for the top-$k$ case in terms of sample complexity, and ran much faster than some of existing BAI-LB algorithms for both top-$k$ and matching cases.


In Chapter~\ref{chap:dense},
the problem of online dense subgraph discovery with linear feedback has been discussed.
We have proposed an $(\epsilon,\delta)$-PAC algorithm called  \textsf{DS-Lin}, and provided a polynomial sample complexity guarantee.
Our key technique was to utilize an approximation algorithm using semidefinite programming (SDP) for confidence bound maximization.
Then, to deal with large-sized graphs, we have proposed an algorithm called \textsf{DS-SR} by combining the successive reject strategy and the greedy peeling algorithm.
We have provided an upper bound of the probability that the quality of the solution obtained by the algorithm is less than $\frac{1}{2}{\rm OPT}-\epsilon$, where OPT is the optimal value.
Computational experiments using well-known real-world graphs have demonstrated the effectiveness of the proposed algorithm. 

In Chapter~\ref{chap:CPE-PL},
the problem of combinatorial pure exploration with partial-linear feedback  has been discussed.
This problem was highly challenging since we should deal with partial-linear feedback and nonlinear reward functions simultaneously in combinatorial action spaces and no existing (even exponential-time) algorithms can solve it.
We have designed the general polynomial-time algorithmic framework \textsf{GCB-PE} with sample complexity analysis.
Our algorithm and its analysis can be applied to any nonlinear reward function with Lipschitz continuity.
The experimental results have shown the superiority of our algorithm in speed, and demonstrated that \textsf{GCB-PE} is the first algorithm which can simultaneously deal with combinatorial action space, partial feedback and nonlinear reward functions.
% There are several interesting directions worth further investigation.
% First, it is open to prove a lower bound of polynomial-time algorithms for both CPE-PL and CPE-BL.
% Another challenging direction is to design efficient algorithms for specific combinatorial cases to choose the global observer set $\sigma$ and the distribution $\lambda^*_{\mathcal{X}_{\sigma}}$, and derive specific sample complexity bounds.
% Furthermore, the extension of CPE-PL to nonlinear feedback is also a practical and valuable problem.
% %\yuko{I added to mention for lower bound}



 \section{Future Directions}
 
 In the final section of this thesis,
 we discuss limitations of the current results and show important subjects for the future.
 While this thesis has focused on the challenges of combinatorial action spaces and limited observation, there are many more, equally important theoretical or real-world challenges that need to be addressed as follows.


 \subsection{Lower Bounds of Polynomial-time $\delta$-PAC Algorithms}

The optimality of the presented sample complexity bounds for full-bandit settings has been discussed by comparing them with the information theoretic lower bounds for the best arm identification in linear bandits (BAI-LB).
We have seen the gap between our sample complexity bounds and the information theoretic lower bounds, and we believe that this gap is needed for reducing computational cost.
To understand whether or not this gap is inevitable for the problems of combinatorial pure exploration, it is important to investigate lower bounds of polynomial-time $\delta$-PAC algorithms.
For the nonlinear rewards or partial-linear feedback, no prior work has provided a lower bound.
Therefore, we have the following future work.

\begin{problem}
Prove a lower bound of polynomial-time algorithms for combinatorial pure exploration problems with full-bandit or partial-linear feedback.
\end{problem}



\subsection{Non-Stationary Environment}
All the studies in this thesis and most existing work focused on the \emph{stationary} case, where the distribution of rewards never changes over time.
However, in real-world applications, we are faced with an extremely \emph{non-stationary} world and it is not reasonable to assume that the distribution stays the same~\citep{besbes2014stochastic}.
For example, in online advertising and recommendation systems,
a user's preferences may likely change when some events happen, which greatly influence the users, and typically exhibit trends on seasonal, weekly, and even daily scales.
Therefore, solving the non-stationary case is promising for increasing the applicability of combinatorial pure exploration methods.

\begin{problem}
Design a method for combinatorial pure exploration problems in non-stationary environments.
\end{problem}



\subsection{Nonlinear Reward Functions and Nonlinear Feedback}
In Chapter~\ref{chap:CPE-PL},
the problem of combinatorial pure exploration with partial-linear feedback for nonliner rewards has been discussed, and  a general polynomial-time algorithmic framework has been given.
However, our algorithm and its analysis are restricted to  nonlinear reward functions that satisfy the Lipschitz continuity, which often fails to hold in practice.
We also considered linear feedback in all previous chapters. 
For a class of reward functions that belong to some reproducing kernel hilbert space (RKHS), \citet{valko2013finite} proposed a kernelized UCB algorithm, and provided a cumulative regret bound.

To discuss this issue more precisely, we will first give the definition of RKHS.
Let $\cH$ be a functional Hilbert space and let $\cD$ be the domain of the functions in $\cH$.
We use ${\langle \cdot, \cdot\rangle}_{\mathcal{H}}$ to denote the inner product in a Hilbert space $\cH$.
The inner product has the following properties for elements $f, g \in \cH$
 and a scalar $a$
 \begin{enumerate}
     \item Linearity: $ {\langle a_1 f_1+a_2 f_2, g\rangle}_{\mathcal{H}} =a_1{\langle  f_1, g\rangle}_{\mathcal{H}} +a_2{\langle f_2, g\rangle}_{\mathcal{H}}$;
     \item Symmetry: $ {\langle f, g\rangle}=\overline{{\langle g, f \rangle}_{\mathcal{H}}}$; 
     \item ${\langle f, f\rangle}_{\mathcal{H}} \geq 0$, ${\langle f, g\rangle}_{\mathcal{H}}=0$ if and only if $f=0$,
 \end{enumerate}
 where $\overline{\cdot}$ denotes the complex conjugate of a scalar.
 

The \emph{reproducing kernel} $K(x,x')$ is a bivariate function defined on $\cD \times \cD$ that satisfies the following conditions.
\begin{enumerate}
    \item For any fixed $x' \in \cD$, $K(x,x')$ belongs to $\cH$ as a function of $x$.
    \item It holds that ${\langle f(\cdot), K(\cdot, x')\rangle}_{\mathcal{H}}=f(x')$ for any $f \in {\mathcal{H}}$, any $x' \in \cD$.
\end{enumerate}
The reproducing kernel has the following properties:
 \begin{enumerate}
     \item  $K(x, x')=\overline{K(x',x)}$ for any $x, x' \in \cD$;
     \item  $K(x, x') \geq 0$ for any $x \in \cD$.
  \end{enumerate}
A Hilbert space that has the reproducing kernel is called a \emph{reproducing kernel Hilbert space}.


In the kernelized linear bandit, we let $\cD=\mathbb{R}^d$ and let an orthonormal basis $\phi$ be the mapping $\phi \mid \mathbb{R}^d \rightarrow \cH$.
Then, we define reproducing kernel function as
\[
K(x,x')=\phi(x)^\top \phi(x') , \quad \forall x, x' \in \mathbb{R}^d.
\]
In the model of~\citet{valko2013finite},
 the existence of $\phi$ is assumed for which there exists $\theta \in \cH$ such that the expected reward for $x \in \cX$ is expressed by $\phi(x)^\top \theta$.
%For non-combinatorial settings, where action size $|\cX|$ xs not so large,
In RKHS,
we can utilize the ridge regression in $\cH$ to build an estimator for $\theta$.
To weaken the assumptions on Lipschitz continuity for reward functions and linear feedback in our model,
we may also consider a wide class of reward functions that belong to RKHS.
In the literature in BAI-LB, no existing work have considered nonlinear reward functions. Thus we may begin with non-combinatorial settings, where action size $|\cX|$ is not so large.

\begin{problem}
Design a method for the best arm identification in kernelized linear bandits.
\end{problem}
Note that $\max_{x\in \cX}\phi(x)^\top \theta$ may be hard since it involves nonconvex optimization.
When $\cX$ is a combinatorial action space, whether or not there still exists a polynomial-time algorithm for finding the optimal arm $x^*=\argmax_{x\in \cX}\phi(x)^\top \theta $ is controversial,
since $\phi(x) \in \mathcal{H}$ may not be a 0--1 vector and thus it is not trivial to utilize combinatorial structures.
% even for some special cases such as the radial basis function kernel $K(x, x')=\exp{(-\|x-x'\|^2/2 \sigma^2)}$ for $\sigma>0$
% and the polynomial kernel $K(x, x')=(x^{\top}x'+1)^p$ for degree $p$.
If such a polynomial-time algorithm is not available in RKHS, we may try to find another class of nonlinear reward functions and devise a specific algorithm to solve it.

\begin{problem}
Devise a method for combinatorial pure exploration with a subclass of nonlinear reward functions.
\end{problem}


%\subsection{Nonlinear Feedback}


% There are several interesting directions worth further investigation.
% First, it is open to 
% Another challenging direction is to design efficient algorithms for specific combinatorial cases to choose the global observer set $\sigma$ and the distribution $\lambda^*_{\mathcal{X}_{\sigma}}$, and derive specific sample complexity bounds.
% Furthermore, the extension of CPE-PL to nonlinear feedback is also a practical and valuable problem.



\subsection{Optimal Experimental Design with Combinatorial Actions}
To investigate the above future work and further improve our current results,
we believe that developing algorithms and theory for the optimal experimental design in combinatorial action spaces is one of the very important topics.
Taking an example of the sample complexity bound provided in Chapter~\ref{chap:CPE-BL},
we will discuss further directions and a connection between pure exploration problems and optimal experimental design.



\paragraph{G-optimal design.}
Some of the BAI-LB algorithms (e.g.~\cite{Soare2014,Tao2018,Fiez2019}) require solving the following G-optimal design problem for their design:
\[
 \min_{\lambda \in \triangle(\cX)}  \max_{x \in \mathcal{X}} \|x\|_{M(\lambda)^{-1}},
\]
where $M(\lambda)^{-1}=\sum_{x \in \mathcal{X}} (\lambda(x) x x^{\top})^{-1}$ is the error covariance matrix.
The G-optimal design aims to minimize the maximum prediction variance, and as shown in \citet{kiefer_wolfowitz_1960}, the continuous G-optimal design and D-optimal design are equivalent when the errors are homoscedastic.
Geometrically, this corresponds to designing the experiment to minimize the volume of the resulting confidence ellipsoid~\citep{boyd2004} (see Figure~\ref{fig:ellipsoid}).
% A design which minimizes the maximum of the standardized variance function
% % over the design region X is called a G-optimal design.
% As shown in \citet{kiefer_wolfowitz_1960}, 
% G-optimal design


%An I-optimal design aims to minimizes the average prediction variance over design space

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{sec/figure/ellipsoid-crop.pdf}
    \caption{The illustration of a confidence ellipsoid, where $X=(x_1, \cdots, x_d)$ is the model matrix. The shape of the ellipsoid depends on the information matrix $X^TX$.}
    \label{fig:ellipsoid}
\end{figure}


The above G-optimal design problem is hard to compute when $|\mathcal{X}|$ is exponentially large, since we have an exponential number of variables and the inner optimization is already hard as discussed in Chapter~\ref{chap:topk}.
%Then, the proposed algorithm  avoids this issue by selecting a set of super arms.
To avoid the high computational cost, the proposed algorithm in Chapter~\ref{chap:CPE-BL}
chose a set of super arms $\mathcal{X}_{\sigma} \subseteq \mathcal{X}$ (the proposed algorithms in  Chapters~\ref{chap:topk} and \ref{chap:dense} also did so).
Then we can obtain 
\[
\lambda^*_\sigma=\argmin_{\lambda \in \triangle(\mathcal{X}_{\sigma} )} \max_{x \in \mathcal{X}_{\sigma}} \|x\|_{M(\lambda)^{-1}},
\]
and guarantee that 
\[
\max_{x \in \mathcal{X}_{\sigma}} \|x\|_{M(\lambda^*_\sigma)^{-1}}=d,
\]
using the theorem in \citet{kiefer_wolfowitz_1960} (see also Proposition~\ref{proposition:equivalence} in Chapter~\ref{chap:CPE-BL}).
Let $m=\max_{x \in \cX} \|x\|^2_2$.
In Lemma~\ref{lemma: alpha} in Chapter~\ref{chap:CPE-BL},
we have already seen that for any $z \in \mathcal{X}$, we have
\begin{align*}
    \|z\|_{M(\lambda^*_\sigma)^{-1}} \leq d \sqrt{m \cdot \xi_{\max}(\widetilde{M}(\lambda^*_{\mathcal{X}_{\sigma}})^{-1})},
\end{align*}
where recall that $\widetilde{M}(\lambda^*_{\mathcal{X}_{\sigma}})=\sum_{x \in \mathrm{supp}(\lambda^*_\sigma)} (x x^{\top})$.
Due to this upper bound,
our sample complexity depends on $\xi_{\max}(\widetilde{M}(\lambda^*_{\mathcal{X}_{\sigma}})^{-1})$.
Therefore, to reduce the sample complexity,
we want to choose a subset $\mathcal{X}_{\sigma} \subseteq \mathcal{X}$ which minimizes
the largest eigenvalue $\xi_{\max}(\widetilde{M}(\lambda^*_{\mathcal{X}_{\sigma}})^{-1})$.
However, such a selection of good super arms corresponds to the \emph{E-optimal design}, i.e., the goal is to minimizing the largest eigenvalue of the error covariance matrix.
This problem is no easier than G-optimal design, which will be discussed in the next paragraph.
We note that in general, 
it seems hard to give an upper bound of 
the largest eigenvalue of the error covariance matrix as the following example for the top-$k$ case implies.
Therefore, we wish to design some efficient methods for the E-optimal design and achieve a better sample complexity.

\begin{example}
We assume that $d$ and $k$ in a given instance of the top-$k$ identification problem  are coprime.
For $i \in [d]$, let the $((i+n) \bmod d)$-th element of $x_i \in \cX$ be $1$ for $n=1,2,\ldots,k$ and other elements of $x_i$ be $0$. Let $\cX_{\sigma}=\{x_1, x_2, \ldots, x_d\} \subseteq \cX$.
Then the information matrix $\sum_{x \in \cX_{\sigma}} (x x^{\top})$ is defined as a following circulant matrix $C$:
\[
C=
\begin{bmatrix}
c_0     & c_{d-1} & \dots  & c_{2} & c_{1}  \\
c_{1} & c_0    & c_{d-1} &         & c_{2}  \\
\vdots  & c_{1}& c_0    & \ddots  & \vdots   \\
c_{d-2}  &        & \ddots & \ddots  & c_{d-1}   \\
c_{d-1}  & c_{d-2} & \dots  & c_{1} & c_0 \\
\end{bmatrix},
\mathrm{where}
\begin{bmatrix}
c_0      \\
c_{1}  \\
\vdots  \\
c_{k-1}\\
c_{k}\\
\vdots\\
c_{d-2k}\\
c_{d-2k+1}\\
\vdots \\
c_{d-2}   \\
c_{d-1}  \\
\end{bmatrix}
=
\begin{bmatrix}
k     \\
k-1\\
\vdots  \\
1   \\
0  \\
\vdots \\
0\\
1\\
\vdots\\
k-2\\
k-1
\end{bmatrix}.
\]
The corresponding eigenvalues are then given by
\begin{align*}
\xi_j = c_0+c_{d-1} \omega_j + c_{d-2} \omega_j^2 + \ldots + c_{1} \omega_j^{n-1}, \qquad j=0,1,\cdots, d-1,
\end{align*}
where $\omega_j=\exp \left(i \tfrac{2\pi j}{d}\right)$ are the $d$-th root of unity and $i$ is the imaginary unit.
\end{example}




\paragraph{E-optimal design.}
% $\max_{X} \lambda_{\min}(X^{\top}X)$ corresponds to so called the {\em E-optimal design}, in which the goal is to minimize the maximum eigenvalue of the error covariance. That is, 

The E-optimal design can be interpreted geometrically as minimizing the diameter of the confidence ellipsoids.
%since the diameter is proportional to the spectral norm $\| (\sum_{x \in \cX} \lambda_x x x^{\top})\|_2$. 
%Let $L$ be is the number of support of $\mathcal{B}$.
Obtaining the E-optimal (discrete) design is known to be NP-hard~\citep{Civril2009},
and the best known result is $(1+\epsilon)$-approximation by \citet{Allen-zhu17e} for $\epsilon>0$.
We remark that existing methods assume $|\mathcal{X}|$ to be small, while $|\mathcal{X}|=O(2^d)$ in our setting~\citep{Allen-zhu17e,Madan19a,pukelsheim2006}.

In the rest of this section,
let $L$ be the number of non-zero elements of $\lambda \in \{0,1\}^{|\mathcal{X}|}$.
The E-optimal design problem with combinatorial action space $\cX$ can be casted as follows.

\begin{alignat*}{4}\label{prob:E-opt} 
& &\ \text{Primal:} \ & \text{minimize} & \  &  \lambda_{\max}\left(\sum_{x_i \in \mathcal{X}} \lambda_i x_i x_i^{\top}\right)^{-1} \notag \\
&              &    &\text{subject to}
%&              &    &\text{subject to} &    & \sum_{i=1}^p \lambda_i x_i x_i ^{\top} \succeq t I \notag \\
 & & \lambda \in \{0,1\}^{|\mathcal{X}|},\  \sum_{x_i \in \mathcal{X}}\lambda_i \leq L.
\end{alignat*}
%   \begin{itembox}[l]{A possible approach and technical issues}
%   Algorithm may look like:\\
%     Step 1. Solve the convex relaxation problem to P1, and obtain the optimal solution $\lambda^*_{c}$.\\
%     Step 2. Obtain approximate solution $\hat{\lambda}$ by some rounding procedure.\\
%     Step 3. Output $\mathcal{B}=\{x_i \mid \lambda_{(x_i)}>0\}$.
    
%     However, the convex relaxation problem is already hard to compute due to exponential number of variables or constraints.

%   \end{itembox}
%with variables $\lambda \in \mathbb{R}^p$ and $t \in \mathbb{R}$.
%This problem is a convex optimization problem.

Relaxing the discrete variables $\lambda \in \{0,1 \}^{|\cX|}$ to continuous one and taking the dual of the relaxation problem, we will obtain the following dual problem.

% The convex relaxation of E-optimal experiment design problem can be formulated as follows~\citep{boyd2004}.
% \begin{alignat*}{4}%\label{prob:E-opt_2} 
% & &\ \text{Primal 2:} \ &\text{minimize} & \  & 1/t \notag \\
% %&              &    &\text{subject to}
% &              &    &\text{subject to} &    & \sum_{x_i \in \mathcal{X}} \lambda_i x_i x_i ^{\top} \succeq t I  \\
%  &&&& & \lambda_i \geq 0,   \ \forall x_i \in \mathcal{X}  \\
%  &&&&&   \sum_{x_i \in \mathcal{X}}\lambda_i \leq L,
% \end{alignat*}
% with variables $\lambda \in \mathbb{R}^{|\mathcal{X}|}$ and $t \in \mathbb{R}$.
% %Notice Primal 2 has the exponential number of variables.
%The dual of the E-optimal design problem can be derived as 
\begin{alignat*}{4}%\label{prob:E-opt_3} 
& &\ \text{Dual 1:} \ &\text{maximize} & \  & \mathrm{Tr}(W)  \notag \\
&              &    &\text{subject to} &    & x_i^{\top} W x_i \leq L, \ \forall x_i \in \mathcal{X} \\
& & & & & W \succeq 0,
\end{alignat*}
with variable $W \in \mathbb{S}_+^d$,
where $\mathbb{S}_+^d$  denotes the
set of symmetric positive semidefinite $d \times  d$ matrices.
The optimal solution $W^*$ determines the minimum volume ellipsoid, centered at the origin, given by $\{x \mid x^{\top}W x \leq L\}$, that contains
the points $x_1, \ldots, x_{|\mathcal{X}|}$.
Due to complementary slackness, 
\begin{align*}
    \lambda^*_i(L-x_i^{\top} W^* x_i)=0 \ \text{for} \ i=1,\ldots,|\mathcal{X}|.
\end{align*}
From the above condition, the optimal design only uses $x_i$ that lies on the surface of the ellipsoid defined by $W^*$.
Notice, however, that
this dual problem still has an exponentially large number of constraints.
We may consider a further relaxation problem.
Let $P(\mathcal{X})$ be a polytope, which is a convex hull of the indicator vectors of all super arms.
\begin{alignat*}{4}%\label{prob:E-opt_4} 
& &\ \text{Dual 2:} \ &\text{maximize} & \  & (W)  \notag \\
&              &    &\text{subject to} &    & x^{\top} W x\leq L, \ \forall x \in P(\mathcal{X}) \\
& & & & & W \succeq 0,
\end{alignat*}
with variable $W \in \mathbb{S}_+^d$.
We can investigate how to solve this problem for specific cases such as matroids or matchings and design a rounding procedure with theoretical guarantee, or take a totally different approach.

To sum up, 
important future work in this line is as follows.
\begin{problem}
Devise a method for optimal experimental design with combinatorial action spaces.
\end{problem}



% \subsection{Directions}
% \begin{itemize}
%     \item Multiplicative weight update method to deal with exponential number of variables? 
%  (However, the constraint (3) is hard to deal with.)
    
%     \item The further relaxation problem?
    
%     \item Methods for the \emph{Semi-Infinite Programming Problem} can be used?
    
%     \item or give up this approach..
% \end{itemize}




% \subsection{Approximation of G-optimal design}

% Tao et al.~\cite{Tao2018} solves the following problem (G-optimal):
% \[
%  \min_{\lambda \in \mathbb{R}^{|\mathcal{X}|} }  \max_{x \in \mathcal{X}} \|x\|_{\sum_{x \in \mathcal{X}} (\lambda(x) x x^{\top})^{-1}}
% \]
% The above problem cannot be solved in our setting since we have exponential size of variables.
% Then, the current algorithm avoid this problem by selecting a set of super-arms.
% However, selecting a good super-arms corresponds to E-optimal design, i.e., the goal is to maximizing the smallest eigenvalues of information matrix.
% This problem is no easier than G-optimal design.



% Also, it is hard to provide examples. Given that, should we back to G-optimal design? Maybe we cannot guarantee $\min_{\lambda \in \mathbb{R}^{|\mathcal{I}|} }  \max_{x \in \mathcal{I}} \|\chi(x)\|_{\sum_{x \in \mathcal{I}} (\lambda(x) \chi(x)chi(x)^{\top})^{-1}}=O(n)$ if it is approximated, but we may show that approximate solution $\lambda_{APX}$ satisfies $Obj(\lambda_{APX}) \leq \beta \times  OPT$ for approximation ratio $\beta=poly(n,k)$.

% \subsection{Approximation algorithm for min max game}
% Mastin et al.~\cite{Mastin2015} addressed the randomized minimax game for combinatorial optimization, in which one player takes a mixed strategy over all feasible solutions,  i.e., $y=(y_S)_{S \in \mathcal{F}}$, where $\mathcal{F}$ is set of all solutions. Similar techniqe can be borrowed to our analysis..?

% We use $\mathcal{F}$ to denote the family of solutions which satisfies a given combinatorial structure.
% Let $\tilde{\mathcal{F}} \subseteq \mathcal{F}$ be the polynomial size subset of  $\mathcal{F}$.
% Let $\triangle(\mathcal{F})$ and $\triangle(\tilde{\mathcal{F}})$ denote the set of probability distributions over a family $\mathcal{F}$ and $\tilde{\mathcal{F}}$.

% Let $r<\frac{1}{|\mathcal{F}|}$ be a positive real.
% Let $w_{S,e}$ be the $e$-th component of the matrix $(\chiS \chiS^T+rI)^{-1}$.
% Let $f_{S}(Y)=\sum_{e \in Y}w_{S,e}$ for $S,Y \in \mathcal{F}$.

% \[
% \min_{q \in \Delta(\mathcal{F})} \max_{Y \in \mathcal{F}} \sum_{X \in \mathcal{I}} q(X) f_X(Y)
% \]



==> sec/short_table.tex <==

\begin{table*}[t]
	\centering
	\caption{Comparison between our results and state-of-the-art results for CPE-BL(PL). ``General'' represents that the algorithm works for any combinatorial structure. $\tilde{O}(\cdot)$ only omits $\log \log$ factors. Main notations are defined in Section~\ref{sec:problem_def}. 
%	A full table and specific notations are given in Appendix~\ref{apx:related_work}. 
	} 
	\label{table:results}
	\renewcommand\arraystretch{1.8}
	\scalebox{0.75}{
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		Algorithm&Sample complexity&Case&Problem Type&Strategy&Time\\
		\hline
		{\bf 
		\textsf{GCB-PE} (ours, Thm.~\ref{thm:GCB_ub})} &$O \big( \frac{ |\sigma| \beta_{\sigma}^2 L_p^2}{\Delta_{\textup{min}}^2} \log \frac{ \beta_{\sigma}^2 L_p^2}{\Delta_{\textup{min}}^2\delta} \big)$& General &CPE-PL&Static&$\mathrm{Poly}(d)$\\
		\hline
		{\bf  
		\textsf{PolyALBA} (ours, Thm.~\ref{thm:CPE-BL})} &$\tilde{O} \big(\sum_{i=2}^{\lfloor \frac{d}{2} \rfloor} \frac{1}{\Delta_i^2} \log \frac{|\mathcal{X}|}{\delta}    +\frac{d^2 m \xi_{\max}({\widetilde{M}({\lambda})}^{-1})}{ \Delta^2_{d+1}} \log \frac{|\mathcal{X}|}{\delta} \big)$&General &CPE-BL& Adaptive  &$\mathrm{Poly}(d)$\\
		\hline
		\textsf{ICB}~\cite{Kuroki+19}&$\tilde{O}\big(\frac{d  \xi_{\max}({M({\lambda})}^{-1})\rho(\lambda)}{\Delta^2_{\min}} \log \frac{d  \xi_{\max}({M({\lambda})}^{-1}) \rho(\lambda)}{\Delta^2_{\min}\delta}\big)$ &General &CPE-BL& Static&$\mathrm{Poly}(d)$\\
%		\hline
%		 \textsf{SAQM}~\cite{Kuroki+19} &$\tilde{O}\big(\frac{d^{1/4}k\xi_{\max}({M({\lambda})}^{-1})\rho(\lambda)}{\Delta_{\min}^2} \log \frac{d^{1/4}k\xi_{\max}({M({\lambda})}^{-1})\rho(\lambda)}{\Delta_{\min}^2  \delta}\big)$ &Top-$k$ &CPE-BL& Static&$\mathrm{Poly}(d)$ \\
		\hline
		\textsf{CSAR}~\cite{Idan2019} &$\tilde{O}\big(\sum^{d}_{i=2}\frac{1}{\tilde{\Delta}_i^2} \log\frac{d}{\delta}\big)$&Top-$k$ &CPE-BL&  Adaptive &$\mathrm{Poly}(d)$ \\
		\hline
%		\textsf{$\mathcal{X}\mathcal{Y}$-static}~\cite{Soare2014}&$O\big(\frac{d}{\Delta_{\textup{min}}^2}\log \frac{|\cX|}{\delta \Delta^2_{\min}} +d^2\big)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Static& $\Omega(|\cX|)$ \\
%		\hline
%		\textsf{\textsf{Explore-Verify}}~\cite{Karin16}&$O\big(\frac{d}{\Delta_{\textup{min}}^2} \log \frac{|\cX|}{\delta \Delta_{\min}}+ d\log \delta^{-1}\big)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Static& $\Omega(|\cX|)$\\
%		\hline
%		\textsf{LinGapE}~\cite{Xu2018}&  $\tilde{O}\big(d  \sum_{x \in \cX} H_x\log \frac{d|\cX|}{\delta} \cdot \sum_{x \in \cX} H_x\big)$ &$\cX \subseteq \mathbb{R}^d$&BAI-LB& Adaptive & $\Omega(|\cX|)$\\
%		\hline
%		$\mathcal{Y}$-\textsf{ElimTil}~\cite{Tao2018}&$\tilde{O}\big(\frac{d}{\Delta_{\textup{min}}^2} (\log \delta^{-1} + \log |\mathcal{X}|)\big)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Adaptive& $\Omega(|\cX|)$\\
%		\hline
	    \textsf{ALBA}~\cite{Tao2018}&$\tilde{O}\big(\sum^{d}_{i=2}\frac{1}{\Delta_i^2}(\log \delta^{-1} + \log |\mathcal{X}|)\big)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Adaptive & $\Omega(|\cX|)$\\
		\hline
		\textsf{RAGE}~\cite{Fiez2019}&$O \big(\sum^{\left \lfloor \log_2(4/\Delta_{\min})  \right \rfloor}_{t=1} 2(2^t)^2\tilde{\rho}(\mathcal{Y}(S_t)) \log(t^2|\mathcal{X}|^2/\delta) \big)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Adaptive& $\Omega(|\cX|)$\\
		\hline
		\textsf{LinGame(-C)} \cite{Degenne+2020}&$\mathop{\lim \sup}_{\delta \rightarrow 0} \frac{\mathbb{E}_{\theta}[\tau_{\delta}]}{\log(1/ \delta)} \leq \min_{\lambda \in \triangle(\cX)}\max_{x\in \mathcal{\cX} \setminus\{x^*\}} \frac{2||x^*-x||_{M(\lambda)^{-1}}^2}{((x^*-x)^{\top}\theta)^2} $&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Adaptive& $\Omega(|\cX|)$ \\
		\hline
		\textsf{Peace} \cite{Katz+2020}&$O\big( (\min_{\lambda \in \triangle(\cX)}\max_{x\in \mathcal{\cX} \setminus\{x^*\}} \frac{||x^*-x||_{M(\lambda)^{-1}}^2}{((x^*-x)^{\top}\theta)^2} + \gamma^* )  \log(1/ \delta)\big)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& Adaptive& $\Omega(|\cX|)$ \\
		\hline
		Lower Bound \cite{Fiez2019}&$\mathbb{E}_{\theta}[\tau_{\delta}] \geq \min_{\lambda \in \triangle(\cX)}\max_{x\in \mathcal{\cX} \setminus\{x^*\}} \frac{||x^*-x||_{M(\lambda)^{-1}}^2}{((x^*-x)^{\top}\theta)^2} \log(1/2.4 \delta)$&$\cX \subseteq \mathbb{R}^d$&BAI-LB& - & - \\
		\hline
	\end{tabular}
	}
\end{table*}

%full-version%

% \begin{table}[h]
% 	\centering
% 	\caption{Comparison between our results and existing results for CPE-PL (BL).
% 	Note that $\Delta_{\min}$ is the minimum reward gap.
% 	The parameter $m$ represents $\max_{x \in \cX} \|x\|_2$, $\delta$ the failure probability. "General" represents any combinatorial constraint in which polynomial-time offline oracle is available with respect to the reward function. Other notations are given in footnotes.}
% 	\scalebox{0.75}{
% 	\begin{tabular}{|c|c|c|c|c|c|}
% 	%\begin{tabular}{|l|l|l|l|l|l|l|}
	
% 		\hline
% 		Algorithm&Sample complexity \footnotemark&Case& $\dfrac{\textup{Reward}}{\textup{Feedback}}$ &Strategy&Time\\
% 		\hline
% 		\textsf{GCB-PE}\footnotemark[2] (Thm.~\ref{thm:GCB_ub}) &$O \left( \frac{ |\sigma| \beta_{\sigma}^2 L_p^2}{\Delta_{\textup{min}}^2} \log\left(\frac{ \beta_{\sigma}^2 L_p^2}{\Delta_{\textup{min}}^2\delta}\right) \right)$&General &  $\dfrac{\mathrm{Nonlinear}}{\mathrm{PL}}$ & Static &$\mathrm{Poly}(d)$\\
% 		\hline
% 		\textsf{EffALBA} (Thm.~\ref{thm:CPE-BL}) &$O \left(\sum_{i=2}^{\lfloor \frac{d}{2} \rfloor} \frac{c_0}{\Delta_i^2} (\log \frac{|\mathcal{X}|}{\delta} \log \Delta_i^{-1})   +\frac{c_0 m^{\frac{3}{2}}d^2 \xi_{\max}({\widetilde{M}_{\lambda}}^{-1})}{ \Delta^2_{d+1}} (\log \frac{|\mathcal{X}|}{\delta} \log \Delta_{d+1}^{-1}) \right)$&General &$\dfrac{\mathrm{Linear}}{\mathrm{BL}}$  & Adaptive  &$\mathrm{Poly}(d)$\\
% 		\hline
% 		\textsf{CSAR}~\cite{Idan2019}\footnotemark[3]  &$O(\sum^{d}_{i=2}\frac{1}{\tilde{\Delta}_i^2}) \log(\frac{d}{\delta})$&Top-$k$ & $\dfrac{\mathrm{Linear}}{\mathrm{BL}}$  &  Adaptive &$\mathrm{Poly}(d)$ \\
% 		\hline
% 		 \textsf{SAQM}~\cite{Kuroki+19} &$O\left(\frac{d^{1/4}k^3\xi_{\max}({M({\lambda})}^{-1})\rho(\lambda)}{\Delta_{\min}^2} (\log \frac{d^{1/4}k^3\xi_{\max}({M({\lambda})}^{-1})\rho(\lambda)}{\Delta_{\min}^2  \delta}+k\log dk\log \frac{d}{\delta})\right)$ &Top-$k$ & $\dfrac{\mathrm{Linear}}{\mathrm{BL}}$  & Static&$\mathrm{Poly}(d)$ \\
% 		\hline
% 		\textsf{ICB}~\cite{Kuroki+19}&$O\left(\frac{d m^2 \xi_{\max}({M({\lambda})}^{-1})\rho(\lambda)}{\Delta^2_{\min}} (\log \frac{d^2 m \xi_{\max}({M({\lambda})}^{-1}) \rho(\lambda)}{\Delta^2_{\min}\delta}+\log d \log \frac{d}{\delta})\right)$ &General & $\dfrac{\mathrm{Linear}}{\mathrm{BL}}$  & Static&$\mathrm{Poly}(d)$\\

% 		\hline
% 		\textsf{$\mathcal{X}\mathcal{Y}$-static}~\cite{Soare2014}&$O\left(\frac{d}{\Delta_{\textup{min}}^2}\left(\log \frac{|\cX|}{\delta}+ \log \Delta^{-1}_{\min} \right)+d^2\right)$&$\cX \subseteq \mathbb{R}^d$&$\dfrac{\mathrm{Linear}}{\mathrm{BL}}$  & Static& $\Omega(|\cX|)$ \\
% 		\hline
% 		\textsf{\textsf{Explore-Verify}}~\cite{Karin16}&$O(\frac{d}{\Delta_{\textup{min}}^2} (\log \frac{|\cX|}{\delta \Delta_{\min}}+ d\log \delta^{-1})$&$\cX \subseteq \mathbb{R}^d$&$\dfrac{\mathrm{Linear}}{\mathrm{BL}}$  & Static& $\Omega(|\cX|)$\\
% 		\hline
% 		\textsf{LinGapE}~\cite{Xu2018}\footnotemark[4]&  $O\left( d \underset{{x \in \cX} }{\sum} H_x\log \frac{d|\cX|}{\delta} \cdot\underset{{x \in \cX} }{\sum} H_x\right)$ &$\cX \subseteq \mathbb{R}^d$&$\dfrac{\mathrm{Linear}}{\mathrm{BL}}$  & Adaptive & $\Omega(|\cX|)$\\
% 		\hline
% 		$\mathcal{Y}$-\textsf{ElimTil}~\cite{Tao2018}&$O(\frac{d}{\Delta_{\textup{min}}^2} (\log \delta^{-1} + \log |\mathcal{X}|+\log\log \Delta^{-1}))$&$\cX \subseteq \mathbb{R}^d$&$\dfrac{\mathrm{Linear}}{\mathrm{BL}}$  & Adaptive& $\Omega(|\cX|)$\\
% 		\hline
% 	    \textsf{ALBA}~\cite{Tao2018}&$O(\sum^{d}_{i=2}\frac{1}{\Delta_i^2}(\log \delta^{-1} + \log |\mathcal{X}|+\log\log \Delta_{i}^{-1}))$&$\cX \subseteq \mathbb{R}^d$&$\dfrac{\mathrm{Linear}}{\mathrm{BL}}$  & Adaptive & $\Omega(|\cX|)$\\
% 		\hline
% 		\textsf{RAGE}~\cite{Fiez2019}\footnotemark[5]&$O \left(\sum^{\left \lfloor \log_2(4/\Delta_{\min})  \right \rfloor}_{t=1} 2(2^t)^2\tilde{\rho}(\mathcal{Y}(S_t)) \log(t^2|\mathcal{X}|^2/\delta) \right)$&$\cX \subseteq \mathbb{R}^d$&$\dfrac{\mathrm{Linear}}{\mathrm{BL}}$  & Adaptive& $\Omega(|\cX|)$\\
% 		\hline
% 		Lower Bound \cite{Fiez2019}&$\min_{\lambda}\max_{z\in \mathcal{Z} \setminus\{z^*\}} \frac{||z^*-z||_{(\sum_{x \in \mathcal{X}} \lambda_x xx^{\top})^{-1}}^2}{((z^*-z)^{\top}\theta^*)^2} \log(1/2.4 \delta)$&$\cX \subseteq \mathbb{R}^d$&$\dfrac{\mathrm{Linear}}{\mathrm{BL}}$  & - & - \\
% 		\hline

% 	\end{tabular}
% 	}
% \end{table}
%\footnotetext{
%	The sample complexity of \textsf{LinGame(-C)} is an asymptotic result.
%	Notations appearing in the table but not relevant in our problem setting are given below:
%$\rho(\lambda)=\max_{x \in \mathcal{X}}\|x\|^2_{M(\lambda)^{-1}}$.
%$\tilde{\Delta}_i=\theta_i - \theta_{k+1}$ if $i \leq k$ and $\theta_k-\theta_i$ otherwise.
%% $H_x=\underset{x_i,x_j \in \cX}{\max}\frac{\bar{\rho}_x(x_i,x_j)}{\max\{\bar{\Delta}^2_i \bar{\Delta}^2_j\}}$  where $\bar{\Delta}=(x^*-x_i)^{\top}\theta$ if $x_i \neq x^*$, $\argmin_{x \in \cX} x^*-x$ otherwise, and $\bar{\rho}_x(x_i,x_j)$ is a term defined by the optimal solution to a convex optimization (see (11) in~\cite{Xu2018}).
% $S_t=\{x \in \cX \mid (x^*-x)^{\top}\theta\leq 4 \cdot 2^{-t} \}$. $\mathcal{Y}(S)=\{ x-x' \mid \forall x,x' \in S, x \neq x'\}$.
%$\tilde{\rho}(\mathcal{Y}(S_t))=\min_{\lambda \in \triangle(\cX)}\max_{v \in \mathcal{Y}(S_t) }\|v\|_{\Mlin}$. 
%$\gamma^*=\min_{\lambda \in \triangle(\cX)} \mathbb{E}_{\eta \sim N(0,1)} \left[ \max_{x\in \mathcal{\cX} \setminus\{x^*\}} \frac{(x^*-x)^\top M(\lambda)^{-1/2} \eta}{(x^*-x)^{\top}\theta} \right]^2. $
%}
% \footnotetext[3]{$\rho^*$ is an information-theoretic lower bound.}


